Geometric flows and the Swampland

After an introductory chapter on the quantum supersymmetric string, in which particular attention will be devoted to the techniques via which phenomenologically viable models can be obtained from the ultraviolet microscopic degrees of freedom, and a brief review of the swampland program, the technical tools required to deal with geometric flows will be outlined. The evolution of a broad family of scalar and metric bubble solutions under Perelman's combined flow will be then discussed, together with their asymptotic behaviour. Thereafter, the geometric flow equations associated to a generalised version of Perelman's entropy function will be derived and employed in defining the action-induced flow associated to a given theory for a scalar field and a dynamical metric. The problem of preserving Einstein field equations along the corresponding moduli space trajectories will be cured by allowing a supplementary energy-momentum tensor term to appear along the flow. In a particular example, such contribution will be shown to precisely reproduce the infinite tower of states with exponentially dropping masses postulated by the distance conjecture.

==> Models/compactifying.tex <==
\begin{equation}\label{actionfinalef2}
\begin{split}
        S&=\frac{1}{2\Bar{\kappa}_{9}^2}\int_\mathcal{P}\diff^{9}x\sqrt{-k}\Biggl\{R_k-\beta^2\frac{56}{49}\left(\nabla\eta\right)^2-\frac{1}{2}\sum_{n\in\Z}\left[\left(\nabla\phi_n\right)^2+e^{-16\beta\eta/7}\frac{n^2}{\rho^2}\phi_n^2\right]\Biggr\}\ .
\end{split}
\end{equation}
Since the Laplacian terms account for nothing more than a boundary term, they were safely removed. We can hence select $\beta$ so that
\begin{equation}
   \frac{56}{49}\beta^2=\frac{1}{2}\Longrightarrow \beta=\sqrt{\frac{7}{16}}
\end{equation}
and obtain the properly rescale Einstein frame action:
\begin{equation}\label{actionfinalef3}
\begin{split}
        S&=\frac{1}{2\Bar{\kappa}_{9}^2}\int_\mathcal{P}\diff^{9}x\sqrt{-k}\Biggl\{R_k-\frac{1}{2}\left(\nabla\eta\right)^2-\frac{1}{2}\sum_{n\in\Z}\left[\left(\nabla\phi_n\right)^2+\frac{n^2}{\rho^2}\phi_n^2e^{-\eta\sqrt{16/7}}\right]\Biggr\}\ .
\end{split}
\end{equation}
Expanding the exponential coupling to $\eta$ as power series, we get:
\begin{equation}
\begin{split}
        e^{-\eta\sqrt{16/7}}\frac{n^2}{\rho^2}\phi_n^2&=\frac{n^2}{\rho^2}\phi_n^2\left(1-\eta\sqrt{\frac{16}{7}}+\frac{16}{7}\eta^2-\dots\right)\ .
\end{split}
\end{equation}

==> Models/dimension.tex <==
\subsubsection{Space-time dimension}
We define a \textit{spurious} state to be a state which is orthogonal to all physical states. Focusing on the NS sector, it can be easily shown, from the physicality conditions \eqref{physcondNS} and the super-Virasoro algebra \eqref{qsupervirasoro}, that such states can always be written as
\begin{equation}
    \ket{\text{spurious}}\equiv L_{-1}\ket{\chi_{-1}}+L_{-2}\ket{\chi_2}\ ,
\end{equation}
where the $\ket{\chi_n}$ satisfy:
\begin{equation}
    \left(L_0-a_0+n\right)\ket{\chi_n}=0\ .
\end{equation}
We define \textit{null} states to be both physical and spurious. In order to construct one, we consider
\begin{equation}
    \ket{\psi}\equiv L_{-1}\ket{\Tilde{\chi}}\ ,
\end{equation}
in which $\ket{\Tilde{\chi}}$ satisfies:
\begin{equation}
    \begin{split}
        \left(L_0-a_0+1\right)\ket{\Tilde{\chi}}&=0\ ,\\
        L_m\ket{\Tilde{\chi}}&=0\quad\text{for}\ m>0\ .
    \end{split}
\end{equation}
Such a state, as pointed out in \cite{Green:2012oqa} and on top of being spurious, almost satisfies the physicality conditions \eqref{physcondNS} in the NS sector. The only non trivial action to be careful about is that of $L_1$, which gives:
\begin{equation}
L_1\ket{\psi}=2L_0\ket{\Tilde{\chi}}=2\left(a_0-1\right)\ket{\Tilde{\chi}}\ .
\end{equation}
Naturally, the above expression is zero if and only if $a_0=1$.

==> Models/extratower.tex <==

We assume the masses to be distributed as:
\begin{equation}
    M_n\left(s\right)\sim\frac{ \Bar{M}_n}{\left[1+\Delta\left(s\right)\right]^\beta}\ ,
\end{equation}
where $\Delta\left(s\right)\equiv\Delta\left(s,0\right)$ is the usual distance and $\beta$ is an order one positive constant. For large flow times, the approximate formula \eqref{distonf2} can be employed and the above scaling translates to:
\begin{equation}
    M_n\left(s\right)\sim \Bar{M}_n\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta} \ .
\end{equation}
Hence, the state with initial mass $M_n\left(0\right)=\Bar{M}_n$ enters the low energy theory, thus contributing to $\Hat{T}$, when we have:
\begin{equation}
    M_n\left(s\right)\leq \Lambda_{\text{EFT}}\ .
\end{equation}
This is approximately achieved at the flow time $s_n$, with:
\begin{equation}
    s_n=\frac{1}{16}\log{\left\{1-\frac{2}{3C_1}\left[1-\left(\frac{\Lambda_{\text{EFT}}}{\Bar{M}_n}\right)^\beta\right]\right\}}\ .
\end{equation}
Assuming, for the sake of the argument, the masses to be distributed according to a relation
\begin{equation}
    \Bar{M}_n\sim\Lambda_{\text{EFT}}\frac{n}{\gamma} 
\end{equation}
inspired by Kaluza-Klein compactification \ref{circlecompactification}, in which the energy scale was singled out and $\gamma$ was introduced to be a constant, we obtain:
\begin{equation}
        s_n=\frac{1}{16}\log{\left\{1-\frac{2}{3C_1}\left[1-\Bigl(\frac{\gamma}{n}\Bigr)^\beta\right]\right\}}\ .
\end{equation}
We can therefore infer that the number of supplementary states which are expected to have entered the theory after a large flow time $s$, thus contributing to $\Hat{T}$, is given by:
\begin{equation}
N\left(s\right)=\gamma\left[1-\frac{3C_1}{2}\left(1-e^{16s}\right)\right]^\beta\ .
\end{equation}
Thus, the overall mass contribution of such states, lying below $\Lambda_{\text{EFT}}$ and appearing in the low energy spectrum at a value $s$ of the flow parameter, is given by:
\begin{equation}
\begin{split}
        M\left(s\right)&=\sum_{n=1}^{N\left(s\right)}M_n\left(s\right)=\sum_{n=1}^{N\left(s\right)}\Bar{M}_n\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta}\\
        &=\frac{\Lambda_{\text{EFT}}}{\gamma}\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta}\sum_{n=1}^{N\left(s\right)}n\\
        &=\frac{\Lambda_{\text{EFT}}}{2\gamma}\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta}N\left(s\right)\Bigl[N\left(s\right)+1\Bigr]\\
        &=\frac{\Lambda_{\text{EFT}}}{2}\left\{\gamma\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^\beta+1\right\}\ .
\end{split}
\end{equation}
For large enough values of the flow parameter, sub-leading terms can be neglected and the above formula can be roughly approximated by:
\begin{equation}
    M\left(s\right)\sim\frac{\gamma\Lambda_{\text{EFT}}}{2}\left[\frac{3C_1}{2}e^{16s}\right]^\beta\ .
\end{equation}
For this to represent the main contribution to the supplementary energy-momentum tensor, we must have
\begin{equation}
    \Hat{T}_{\mu\nu}\left(s\right)\sim-\frac{M^2\left(s\right)}{2}\phi^2\left(s\right)
\end{equation}

==> Models/fromaction.tex <==
\label{gfa}
The introduction of entropy functional, at first in the standard form considered in \eqref{Perelentropy} and then with the more general expression \eqref{funk}, allowed us to derive a set geometric flow equations for a system comprised of a dynamical metric tensor and a scalar field, instead of simply postulating them. While representing a significant achievement, this new conceptual framework might arguably not be regarded as satisfying from the perspective of physics. At a close inspection, part of the arbitrariness which was previously exerted in the specification of a geometric flow was simply pushed to the choice of an entropy functional. Therefore, we now want to start from a particular space-time theory for a $D$-dimensional metric and a scalar, provided with an appropriate dynamics, and use it to completely determine a set of geometric flow equations. By doing so, we will get rid of the above mentioned arbitrariness and exploit the one functional that physics already grants us with: the action. In practice, this will translate into taking the Einstein frame action for a theory, moving to string frame and treating the resulting expression for the action as an entropy functional, from which a set of geometric flow equations will be obtained. We hence start from the Lorentzian dynamics governed by
\begin{equation}\label{aact}
    \tilde{S}\left[\tilde{g},f\right]=\frac{1}{2\kappa^2_D}\int_{\mathcal{M}}\diff^{D}x\sqrt{-\tilde{g}}\left[R_{\tilde{g}}+\frac{1}{2}\left(\nabla f\right)^{2}+\sum_{n=0}^{\infty}\frac{g_{n}}{n!}f^{n}\right]
\end{equation}
and rescale both the metric $\tilde{g}$ and the scalar $f$, in order to obtain the string frame expression for \eqref{aact}. We thus introduce the fields $g$ and $\phi$, associated to the previous ones by:
\begin{equation}
    \tilde{g}_{\mu\nu}\equiv e^{2\varphi}g_{\mu\nu},\quad f\equiv\sigma\phi\ .
\end{equation}
Under such redefinition of the dynamical degrees of freedom, the action \eqref{aact} becomes:
\begin{equation}\label{sfaact}
\begin{split}
        S\left[g,\phi\right]&\equiv\frac{1}{2\kappa^2_D}\int_{\mathcal{M}}\diff^{D}x\sqrt{-g}e^{\left(D-2\right)\varphi}\biggl[R_g-\left(D-2\right)\left(D-1\right)\left(\nabla\varphi\right)^2\\
     &\quad\quad\quad\quad\quad\quad-2\left(D-1\right)\nabla^2\varphi+\frac{\sigma^{2}}{2}\left(\nabla\phi\right)^{2}+e^{2\varphi}\sum_{n=0}^{\infty}\frac{\sigma^{n}g_{n}}{n!}\phi^{n}\biggr]\ .
\end{split}
\end{equation}
For the volume element to take the appropriate string frame form, we take:
\begin{equation}
    \varphi\equiv\frac{1}{2-D}\phi\ .
\end{equation}
Therefore, we obtain:
\begin{equation}\label{sfact2}
\begin{split}
        S\left[g,\phi\right]&\equiv\frac{1}{2\kappa^2_D}\int_{\mathcal{M}}\diff^{D}x\sqrt{-g}e^{-\phi}\biggl[R_g+\left(\frac{\sigma^{2}}{2}-\frac{D-1}{D-2}\right)\left(\nabla\phi\right)^2\\
     &\quad\quad\quad\quad\quad\quad+2\frac{D-1}{D-2}\nabla^2\phi+\exp{\frac{2\phi}{2-D}}\sum_{n=0}^{\infty}\frac{\sigma^{n}g_{n}}{n!}\phi^{n}\biggr]\ .
\end{split}
\end{equation}
The constant $\sigma$ can be fixed by imposing
\begin{equation}
    \frac{\sigma^{2}}{2}-\frac{D-1}{D-2}=1\Longrightarrow \sigma=\sqrt{\frac{4D-6}{D-2}}\ .
\end{equation}
so that the expression \eqref{sfact2} can be more easily connected with Perelman's original $\mathcal{F}$-functional. We are therefore left with:
\begin{equation}\label{sfact2}
\begin{split}
        S\left[g,\phi\right]&\equiv\frac{1}{2\kappa^2_D}\int_{\mathcal{M}}\diff^{D}x\sqrt{-g}e^{-\phi}\Biggl[R_g+\left(\nabla\phi\right)^2+2\frac{D-1}{D-2}\nabla^2\phi\\
     &\quad\quad\quad\quad\quad\quad+\exp{\frac{2\phi}{2-D}}\sum_{n=0}^{\infty}\frac{g_{n}}{n!}\phi^{n}\left(\frac{4D-6}{D-2}\right)^{n/2}\Biggr]\ .
\end{split}
\end{equation}
The above expression can be made simpler by defining the constants
\begin{equation}
    p\equiv\frac{2}{2-D},\quad q_{n}\equiv\frac{g_{n}}{n!}\left(\frac{4D-6}{D-2}\right)^{n/2}
\end{equation}
and observing that:
\begin{equation}
    e^{p\phi}\sum_{n=0}^{\infty}q_n\phi^n=\sum_{n=0}^{\infty}\phi^n\sum_{k=0}^{n}\frac{g_{k}}{\left(n-k\right)!k!}\left(\frac{4D-6}{D-2}\right)^{\frac{k}{2}}\left(\frac{2}{2-D}\right)^{n-k} \ .
\end{equation}
Therefore, by defining
\begin{equation}
    s_{\ n}^{(D)}\equiv\sum_{k=0}^{n}\frac{g_{k}}{\left(n-k\right)!k!}\left(\frac{4D-6}{D-2}\right)^{\frac{k}{2}}\left(\frac{2}{2-D}\right)^{n-k}
\end{equation}
for $n\geq 0$, the string frame action takes the following form:
\begin{equation}\label{entract}
     S\left[g,\phi\right]=\frac{1}{2\kappa^2_D}\int_{\mathcal{M}}\diff^{D}x\sqrt{-g}e^{-\phi}\Biggl[R_g+\left(\nabla \phi\right)^2+2\frac{D-1}{D-2}\nabla^2\phi+\sum_{n=0}^{\infty}s_{\ n}^{(D)}\phi^{n}\Biggr]\ .
\end{equation}
Hence, starting from the space-time action \eqref{aact} and moving to string frame, we have obtained a functional over the generalised moduli space $\mathbf{\Gamma}_{\mathcal{M}}$ that falls into the general class described by \eqref{funk}. More specifically, it corresponds to the choice of:
\begin{equation}
    \alpha=1,\quad\gamma=2\frac{D-1}{D-2},\quad\beta_{n}=s_{\ n}^{(D)}\ .
\end{equation}
The set of geometric flow equations induced by \eqref{entract} for $g$ and $\phi$, which can be obtained by plugging the above constant into the general formulas \eqref{geneq}, are:
\begin{equation}\label{acteq}
\begin{split}
        \frac{\diff g_{\mu\nu}}{\diff s}&=-2R_{\mu\nu}-4\frac{D-1}{D-2}\nabla_\mu\phi\nabla_\nu\phi+\sum_{n=1}^{\infty}ns_{\ n}^{(D)}\phi^{n-1}g_{\mu\nu}\\
        &\quad+4\frac{D-1}{D-2}\bigl[\left(\nabla\phi\right)^2-\nabla^2\phi\bigr]g_{\mu\nu}+\mathcal{L}_\xi g_{\mu\nu}\ ,\\
        \frac{\diff\phi}{\diff s}&=-R+\frac{D\left(2D-3\right)}{D-2}\left(\nabla\phi\right)^2+\frac{D}{2}\sum_{n=1}^{\infty}ns_{\ n}^{(D)}\phi^{n-1}\\
        &\quad-\frac{D\left(2D-1\right)-2}{D-2}\nabla^2\phi+\mathcal{L}_\xi\phi\ .
\end{split}
\end{equation}
Starting from the $D$-dimensional Lorentzian action for a system comprised of dynamical metric and a scalar field, in which the latter is subject to arbitrary polynomial self interactions, and treating its string frame expression as an entropy functional of the form presented in \eqref{funk}, we have derived a set of geometric flow equations without the necessity of postulating some additional, arbitrary structure.  

==> Models/keepingonshell.tex <==
\subsubsection{Keeping the flow on-shell}
In order to address the issue of preserving the on-shell conditions for the metric along the flow in a general setting, we would have to compute the tensors $B_{\mu\nu}$ and $E_{\mu\nu}$ whose properties were discussed in \eqref{act-inon}. In this case, nonetheless, the flow has already been solved numerically. Even more interestingly, it has been provided with an analytic approximation in the large $s$ regime. We can hence directly study the flow behaviour of the energy-momentum tensor $\Bar{T}_{\mu\nu}$ from those of the scalar field and the geometry, impose Einstein field equations not to be broken by the flow and read off the form of the additional energy-momentum contribution $\Hat{T}_{\mu\nu}$. As far as $\Bar{T}_{\mu\nu}$ is concerned, we obtain:
\begin{equation}
    \kappa_4^2\Bar{T}_{\mu\nu}\left(s\right)=\left[\phi^2\left(s\right)-\frac{1}{2}\phi^4\left(s\right)\right]g_{\mu\nu}\left(s\right)\ .
\end{equation}
Focusing on its trace, which will be enough for the present analysis, we are left with:
\begin{equation}
    \kappa_4^2\Bar{T}\left(s\right)=2\phi^2\left(s\right)\left[2-\phi^2\left(s\right)\right]\ .
\end{equation}
On the other hand, we have that the scalar curvature $R$ flows as previously described. It is obvious that, for the geometry to be on-shell along the flow, the trace of the additional energy-momentum contribution must satisfy
\begin{equation}
    R\left(s\right)=-\kappa^2_4\left[\Bar{T}\left(s\right)+\Hat{T}\left(s\right)\right]\ .
\end{equation}
for every value of the flow parameter $s$. Therefore, we have:
\begin{equation}
    \kappa^2_4\Hat{T}\left(s\right)=2\phi^2\left(s\right)\left[\phi^2\left(s\right)-2\right]-R\left(s\right)\ .
\end{equation}
For large values of the flow parameter $s$, the above expression is approximated by:
\begin{equation}\label{flowaddem}
    \kappa^2_4\Hat{T}\left(s\right)\sim 2C_1^4\exp{64s}\ .
\end{equation}
The additional energy-momentum tensor term, included for the flow to keep the geometry on-shell, displays an exponential blow up for large enough values of the flow parameter. Let's now assume that the theory we are dealing with is defined below a certain energy cut-off $\Lambda_{\text{EFT}}$, above which its effective description breaks down. If the supplementary energy-momentum contribution is really to be interpreted as coming from an infinite tower of new states, getting exponentially lighter along the flow, then those must lie above $\Lambda_{\text{EFT}}$ at the beginning of the flow. This is consistent with $\Hat{T}=0$. Moreover, the $s$ dependence in \eqref{flowaddem} should be accounted for by the progressive appearance of states in the effective descriptions, as their masses decrease and cross the energy cut-off. Labelling such fields as $\phi_n$, the swampland distance conjecture suggests that their masses should be controlled by
\begin{equation}\label{expdrop}
    M_n\left(s\right)\sim \Bar{M}_ne^{-\beta\cdot\Delta\left(s\right)}\ ,
\end{equation}
where $\Delta\left(s\right)\equiv\Delta\left(s,0\right)$ is the usual distance and $\beta$ is an order one positive constant. Nonetheless, it must not be neglected that the behaviour described above should be characteristic of superstring low energy effective field theories, as widely discussed in \ref{sec:distanceconj}. There are, indeed, strong arguments \cite{Basile:2022sda} hinting at the fact that the typical exponential drop \eqref{expdrop} should solely be encountered in such scenarios, while towers emerging in apparently consistent theories not coming from superstrings should display power law decays in the distance. There is hence no reason to believe that a generic solution, as the one constructed in the current section, should be characterised by a tower of asymptotically massless states precisely fulfilling \eqref{expdrop}. It would, instead, be the case if and only if our original construction, with a quartic potential \eqref{6pot}, belonged to the string theory landscape. At the same time, imposing the geometry to always be on-shell already provided us with an explicit formula for the flow behaviour of the additional energy-momentum tensor term, precisely associated to the tower of states. This, subsequently, poses a strong constraint on the flow behaviour of their masses. An incompatibility between such a constraint and an exponential drop of the form outlined in \eqref{expdrop} could, hence, be interpreted as a signal of our original $4$-dimensional theory not belonging to the landscape in the first place. We will therefore compare the results produced by an ansatz \eqref{expdrop} and one characterised by a \textit{power-law} decay in the distance, assessing which one correctly delivers the energy-momentum contribution described by \eqref{flowaddem}. In order to do so, we will assume the fields in the tower to be space-time constant, equal to each other, free and not to change along the flow, so that the only relevant flowing quantities will be their masses.
\paragraph{Exponential decay ansatz}
First of all, as previously anticipated, we focus on an exponential ansatz as the one presented in \eqref{expdrop}. For large flow times, the approximate formula \eqref{distonf2} can be employed and such a scaling translates to:
\begin{equation}
    M_n\left(s\right)\sim \Bar{M}_n\exp{\frac{3C_1}{2}\left(1-e^{16s}\right)\beta}\ .
\end{equation}
Hence, the state with initial mass $M_n\left(0\right)=\Bar{M}_n$ enters the low energy theory, thus contributing to $\Hat{T}$, when we have:
\begin{equation}
    M_n\left(s\right)\leq \Lambda_{\text{EFT}}\ .
\end{equation}
This is approximately achieved at the flow time $s_n$, with:
\begin{equation}
    s_n\equiv\frac{1}{16}\log{\left(1-\frac{2}{3C_1\beta}\log{\frac{\Lambda_{\text{EFT}}}{\Bar{M}_n}}\right)}\ .
\end{equation}
Assuming, for the sake of the argument, the masses to be distributed according to a relation

\begin{equation}
    \Bar{M}_n\sim\Lambda_{\text{EFT}}\frac{n}{\gamma} 
\end{equation}
inspired by Kaluza-Klein compactification \ref{circlecompactification}, in which the energy scale was singled out and $\gamma$ was introduced to be a constant, we obtain:
\begin{equation}
    s_n=\frac{1}{16}\log{\left(1+\frac{2}{3C_1\beta}\log{\frac{n}{\gamma}}\right)}\ .
\end{equation}
We can therefore infer that the number of supplementary states which are expected to have entered the theory after a large flow time $s$, thus contributing to $\Hat{T}$, is given by:
\begin{equation}
    N\left(s\right)=\gamma\exp{\frac{3C_1}{2}\left(e^{16s}-1\right)\beta}\ .
\end{equation}
Thus, the overall mass contribution of such states, lying below $\Lambda_{\text{EFT}}$ and appearing in the low energy spectrum at a value $s$ of the flow parameter, is given by:
\begin{equation}
\begin{split}
        M\left(s\right)&=\sum_{n=1}^{N\left(s\right)}M_n\left(s\right)=\sum_{n=1}^{N\left(s\right)}\Bar{M}_n\exp{\frac{3C_1}{2}\left(1-e^{16s}\right)\beta}\\
        &=\frac{\Lambda_{\text{EFT}}}{\gamma}\exp{\frac{3C_1}{2}\left(1-e^{16s}\right)\beta} \sum_{n=1}^{N\left(s\right)}n\\
        &=\frac{\Lambda_{\text{EFT}}}{2\gamma}\exp{\frac{3C_1}{2}\left(1-e^{16s}\right)\beta}N\left(s\right)\bigl[N\left(s\right)+1\bigr]\\
        &=\frac{\Lambda_{\text{EFT}}}{2}\left\{\gamma\exp{\frac{3C_1}{2}\left(e^{16s}-1\right)\beta}+1\right\}\ .
\end{split}
\end{equation}
For large enough values of the flow parameter, sub-leading terms can be neglected and the above formula can be roughly approximated by:
\begin{equation}
    M\left(s\right)\sim\frac{\gamma\Lambda_{\text{EFT}}}{2}\exp{\frac{3C_1\beta}{2}e^{16s}}
\end{equation}
For these masses to represent the main contribution to the supplementary energy-momentum tensor, we must have:
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim-\sum_{n=1}^{N\left(s\right)}M^2_n\left(s\right)\cdot\phi^2_n\left(s\right)=-\sum_{n=1}^{N\left(s\right)}\Bar{M}^2_n\exp{3C_1\beta\left(1-e^{16s}\right)}\cdot\phi^2_n\left(s\right)\\
        &=-\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\right)^2\exp{3C_1\beta\left(1-e^{16s}\right)}\sum_{n=1}^{N\left(s\right)}n^2\cdot\phi^2_n\left(s\right)\ .
\end{split}
\end{equation}
The simple possible ansatz, now, is to take all fields to converge to the same long term value. This can be naturally achieved by requiring
\begin{equation}
    \phi_n\left(s\right)\sim \Hat{\phi}
\end{equation}
for large values of the flow parameter $s$. With such an assumption, the above expression simply turns to: 
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim-\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\Hat{\phi}\left(s\right)\right)^2\exp{3C_1\beta\left(1-e^{16s}\right)}\sum_{n=1}^{N\left(s\right)}n^2\\
        &=-\frac{1}{6}\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\Hat{\phi}\right)^2\exp{3C_1\beta\left(1-e^{16s}\right)}\cdot\Bigl[2N^3\left(s\right)+3N^2\left(s\right)+N\left(s\right)\Bigr]\ .
\end{split}
\end{equation}
Neglecting sub-leading terms, we have:
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim-\frac{1}{3}\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\Hat{\phi}\right)^2\exp{-3C_1\beta e^{16s}}\cdot N^3\left(s\right)\\
        &=-\frac{\gamma}{3}\left(\Lambda_{\text{EFT}}\cdot\Hat{\phi}\right)^2\exp{\frac{3C_1\beta}{2}e^{16s}}\ .
\end{split}
\end{equation}
Such a behaviour cannot be matched to \eqref{flowaddem}, not allowing an exponential decay in the masses of the $\phi_n$ states while keeping the geometry on shell. Therefore, our original quartic scalar field theory, if left unchanged, cannot be part of the superstring landscape.

\paragraph{Power-law decay ansatz}
In the following discussion, after having assessed that an exponential mass drop is prohibited by the on-shell condition, we assume the masses to display a power-law decay:
\begin{equation}
    M_n\left(s\right)\sim\frac{ \Bar{M}_n}{\left[1+\Delta\left(s\right)\right]^\beta}\ ,
\end{equation}
where $\Delta\left(s\right)\equiv\Delta\left(s,0\right)$ is the usual distance and $\beta$ is an order one positive constant. For large flow times, the approximate formula \eqref{distonf2} can be employed and the above scaling translates to:
\begin{equation}
    M_n\left(s\right)\sim \Bar{M}_n\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta} \ .
\end{equation}
Hence, the state with initial mass $M_n\left(0\right)=\Bar{M}_n$ enters the low energy theory, thus contributing to $\Hat{T}$, when we have:
\begin{equation}
    M_n\left(s\right)\leq \Lambda_{\text{EFT}}\ .
\end{equation}
This is approximately achieved at the flow time $s_n$, with:
\begin{equation}
    s_n=\frac{1}{16}\log{\left\{1-\frac{2}{3C_1}\left[1-\left(\frac{\Lambda_{\text{EFT}}}{\Bar{M}_n}\right)^\beta\right]\right\}}\ .
\end{equation}
Assuming, once again, the masses to be distributed according to a relation
\begin{equation}
    \Bar{M}_n\sim\Lambda_{\text{EFT}}\frac{n}{\gamma} 
\end{equation}
inspired by Kaluza-Klein compactification \ref{circlecompactification}, we obtain:
\begin{equation}
        s_n=\frac{1}{16}\log{\left\{1-\frac{2}{3C_1}\left[1-\Bigl(\frac{\gamma}{n}\Bigr)^\beta\right]\right\}}\ .
\end{equation}
We can therefore infer that the number of supplementary states which are expected to have entered the theory after a large flow time $s$, thus contributing to $\Hat{T}$, is given by:
\begin{equation}
N\left(s\right)=\gamma\left[1-\frac{3C_1}{2}\left(1-e^{16s}\right)\right]^\beta\ .
\end{equation}
Thus, the overall mass contribution of such states, lying below $\Lambda_{\text{EFT}}$ and appearing in the low energy spectrum at a value $s$ of the flow parameter, is given by:
\begin{equation}
\begin{split}
        M\left(s\right)&=\sum_{n=1}^{N\left(s\right)}M_n\left(s\right)=\sum_{n=1}^{N\left(s\right)}\Bar{M}_n\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta}\\
        &=\frac{\Lambda_{\text{EFT}}}{\gamma}\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta}\sum_{n=1}^{N\left(s\right)}n\\
        &=\frac{\Lambda_{\text{EFT}}}{2\gamma}\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta}N\left(s\right)\Bigl[N\left(s\right)+1\Bigr]\\
        &=\frac{\Lambda_{\text{EFT}}}{2}\left\{\gamma\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^\beta+1\right\}\ .
\end{split}
\end{equation}
For large enough values of the flow parameter, sub-leading terms can be neglected and the above formula can be roughly approximated by:
\begin{equation}
    M\left(s\right)\sim\frac{\gamma\Lambda_{\text{EFT}}}{2}\left[\frac{3C_1}{2}e^{16s}\right]^\beta\ .
\end{equation}
For these masses to represent the main contribution to the supplementary energy-momentum tensor, we must satisfy the following identity:
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim-\sum_{n=1}^{N\left(s\right)}M^2_n\left(s\right)\cdot\phi^2_n\left(s\right)=-\sum_{n=1}^{N\left(s\right)}\Bar{M}^2_n\phi^2_n\left(s\right)\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-\beta}\ .
\end{split}
\end{equation}
By once more taking
\begin{equation}
    \phi_n\left(s\right)\sim \Hat{\phi}
\end{equation}
for large values of the flow parameter $s$, we obtain:
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim-\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\Hat{\phi}\right)^2\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-2\beta}\sum_{n=1}^{N\left(s\right)}n^2\\
        &=-\frac{1}{6}\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\Hat{\phi}\right)^2\Bigl[2N^3\left(s\right)+3N^2\left(s\right)+N\left(s\right)\Bigr]\cdot\left[1+\frac{3C_1}{2}\left(e^{16s}-1\right)\right]^{-2\beta}\ .
\end{split}
\end{equation}
By neglecting all sub-leading terms, we have:
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim-\frac{1}{3}\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\Hat{\phi}\right)^2N^3\left(s\right)\cdot\left[\frac{3C_1}{2}e^{16s}\right]^{-2\beta}\\
        &=-\frac{\gamma}{3}\left(\Lambda_{\text{EFT}}\cdot\Hat{\phi}\right)^2\cdot\left[\frac{3C_1}{2}e^{16s}\right]^{\beta}\ .
\end{split}
\end{equation}
By matching the above expression to \eqref{flowaddem} and setting $\beta=4$, we get:
\begin{equation}
2=-\frac{\gamma}{3}\left(\Lambda_{\text{EFT}}\cdot\Hat{\phi}\right)^2\cdot\left(\frac{3}{2}\right)^4\ .
\end{equation}

%State as a conjecture
%Maybe, add an example from circle compactified strings





==> Models/kkkkkk.tex <==

Hence, the state with initial mass $M_n\left(0\right)=\Bar{M}_n$ enters the low energy theory, thus contributing to $\Hat{T}$, when we have:
\begin{equation}
    M_n\left(s\right)\leq \Lambda_{\text{EFT}}\ .
\end{equation}
This is approximately achieved at the flow time $s_n$, with:
\begin{equation}
    s_n\equiv\frac{1}{16}\log{\left(1-\frac{2}{3C_1\beta}\log{\frac{\Lambda_{\text{EFT}}}{\Bar{M}_n}}\right)}\ .
\end{equation}
Assuming, for the sake of the argument, the masses to be distributed according to a relation

\begin{equation}
    \Bar{M}_n\sim\Lambda_{\text{EFT}}\frac{n}{\gamma} 
\end{equation}
inspired by Kaluza-Klein compactification \ref{circlecompactification}, in which the energy scale was singled out and $\gamma$ was introduced to be a constant, we obtain:
\begin{equation}
    s_n=\frac{1}{16}\log{\left(1+\frac{2}{3C_1\beta}\log{\frac{n}{\gamma}}\right)}\ .
\end{equation}
We can therefore infer that the number of supplementary states which are expected to have entered the theory after a large flow time $s$, thus contributing to $\Hat{T}$, is given by:
\begin{equation}
    N\left(s\right)=\gamma\exp{\frac{3C_1}{2}\left(e^{16s}-1\right)\beta}\ .
\end{equation}
Thus, the overall mass contribution of such states, lying below $\Lambda_{\text{EFT}}$ and appearing in the low energy spectrum at a value $s$ of the flow parameter, is given by:
\begin{equation}
\begin{split}
        M\left(s\right)&=\sum_{n=1}^{N\left(s\right)}M_n\left(s\right)=\sum_{n=1}^{N\left(s\right)}\Bar{M}_n\exp{\frac{3C_1}{2}\left(1-e^{16s}\right)\beta}\\
        &=\frac{\Lambda_{\text{EFT}}}{\gamma}\exp{\frac{3C_1}{2}\left(1-e^{16s}\right)\beta} \sum_{n=1}^{N\left(s\right)}n\\
        &=\frac{\Lambda_{\text{EFT}}}{2\gamma}\exp{\frac{3C_1}{2}\left(1-e^{16s}\right)\beta}N\left(s\right)\bigl[N\left(s\right)+1\bigr]\\
        &=\frac{\Lambda_{\text{EFT}}}{2}\left\{\gamma\exp{\frac{3C_1}{2}\left(e^{16s}-1\right)\beta}+1\right\}\ .
\end{split}
\end{equation}
For large enough values of the flow parameter, sub-leading terms can be neglected and the above formula can be roughly approximated by:
\begin{equation}
    M\left(s\right)\sim\frac{\gamma\Lambda_{\text{EFT}}}{2}\exp{\frac{3C_1\beta}{2}e^{16s}}
\end{equation}
In order to compute the energy momentum contribution of such towers of fields, we must first provide them with simple functional forms. In particular, we assume the equations of motion
\begin{equation}
    \left(\nabla^2-M_n^2\right)\phi_n=0
\end{equation}
to be satisfied along the flow. The minus sign appearing in front of the squared mass is consistent with our signature choice. Since the geometry asymptotically approaches that of Minkowski space-time, we have that
\begin{equation}
    \left(\de^2-M_n^2\right)\phi_n\sim 0
\end{equation}
for large values of the flow time $s$. A simple solution to the above equation is given by outgoing massive waves
\begin{equation}
    \phi_n\sim A_n\exp{-iM_nk_\mu x^\mu}\ ,
\end{equation}
in which $k_\mu$ is a unit direction vector. Hence, the overall energy-momentum tensor contribution of such states is given, for large values of the flow parameter, by:
\begin{equation}
    \kappa_4^2 \Tilde{T}_{\mu\nu}=\frac{1}{2}\sum_{n=1}^{N\left(s\right)}\de_\mu \phi_n\de_\nu \phi_n - \frac{1}{4}\sum_{n=1}^{N\left(s\right)}\left[\left(\de \phi_n\right)^{2}+M_n^2\phi_n^{2}\right]g_{\mu\nu}\ .
\end{equation}
Focusing on its trace, we are left with:
\begin{equation}
    \kappa_4^2 \Tilde{T}= - \sum_{n=1}^{N\left(s\right)}\left[\frac{1}{2}\left(\de \phi_n\right)^{2}+M_n^2\phi_n^{2}\right]\ .
\end{equation}




For these masses to represent the main contribution to the supplementary energy-momentum tensor, we must have:
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim-\sum_{n=1}^{N\left(s\right)}M^2_n\left(s\right)\cdot\phi^2_n\left(s\right)=-\sum_{n=1}^{N\left(s\right)}\Bar{M}^2_n\exp{3C_1\beta\left(1-e^{16s}\right)}\cdot\phi^2_n\left(s\right)\\
        &=-\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\right)^2\exp{3C_1\beta\left(1-e^{16s}\right)}\sum_{n=1}^{N\left(s\right)}n^2\cdot\phi^2_n\left(s\right)\ .
\end{split}
\end{equation}
The simple possible ansatz, now, is to take all fields to converge to the same long term evolution. This can be naturally achieved by requiring
\begin{equation}
    \phi_n\left(s\right)\sim \Hat{\phi}\left(s\right)
\end{equation}
for large values of the flow parameter $s$. With such an assumption, the above expression simply turns to: 
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim-\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\Hat{\phi}\left(s\right)\right)^2\exp{3C_1\beta\left(1-e^{16s}\right)}\sum_{n=1}^{N\left(s\right)}n^2\\
        &=-\frac{1}{6}\left(\frac{\Lambda_{\text{EFT}}}{\gamma}\Hat{\phi}\left(s\right)\right)^2\exp{3C_1\beta\left(1-e^{16s}\right)}\\
        &\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\cdot N\left(s\right)\cdot\Bigl[N\left(s\right)+1\Bigr]\cdot\Bigl[2N\left(s\right)+1\Bigr]
\end{split}
\end{equation}
The simple possible ansatz, now, is to take all fields to equally contribute to the energy-momentum tensor. This can be naturally achieved by requiring
\begin{equation}
    \phi_n\left(s\right)\sim\frac{C_2}{n}\Hat{\phi}\left(s\right)
\end{equation}
for large values of the flow parameter $s$, with $C_2$ being a real constant. With such an assumption, the above expression simply turns to:
\begin{equation}
\begin{split}
        \kappa^2_4\Hat{T}\left(s\right)&\sim -\left(\frac{C_2\Lambda_{\text{EFT}}}{\gamma}\right)^2\exp{3C_1\beta\left(1-e^{16s}\right)}N\left(s\right)\cdot\Hat{\phi}^2\left(s\right)\\
        &=-\left(\frac{C_2\Lambda_{\text{EFT}}}{\gamma}\right)^2\exp{3C_1\beta\left(1-e^{16s}\right)}\gamma\exp{\frac{3C_1}{2}\left(e^{16s}-1\right)\beta}\cdot\Hat{\phi}^2\left(s\right)
\end{split}
\end{equation}



\newpage
As far as the distance formula is concerned, we can once more factor out the volume term, as was done in \ref{quart}, and obtain
\begin{equation}
    \Delta\left(s,s_0\right)=\log{\frac{\mathcal{T}\left(s_0\right)}{\mathcal{T}\left(s\right)}}\ ,
\end{equation}
in which we have introduced:
\begin{equation}
\begin{split}
        \mathcal{T}\left(s\right)&=e^{-\phi\left(s\right)}\left(R\left(s\right)-\sum_{n=0}^{\infty}s_{\ n}^{(4)}\phi^{n}\left(s\right)\right)\\
        &=e^{-\phi\left(s\right)}\left\{R\left(s\right)-\frac{V_0}{\alpha_0}\left[\phi^6\left(s\right)-9\phi^4\left(s\right)+21\phi^2\left(s\right)\right]e^{-\phi\left(s\right)}\right\}\ .
\end{split}
\end{equation}
\begin{equation}
    s_{\ n}^{(4)}=\sum_{k=0}^{n}\left(-1\right)^{n-k}\frac{g_{k}}{\left(n-k\right)!k!}
\end{equation}
\begin{equation}
    g_{2}=42\frac{V_0}{\alpha_0}\ ,\quad g_{4}=-9\cdot 4!\frac{V_0}{\alpha_0}\ ,\quad g_{6}=6!\frac{V_0}{\alpha_0}\ .
\end{equation}
The coefficients are:
\begin{equation}
    \begin{split}
        s_{\ 0}^{(4)}&=s_{\ 1}^{(4)}=0\ ,\quad s_{\ 2}^{(4)}=21\frac{V_0}{\alpha_0}\ ,\quad s_{\ 3}^{(4)}=-21\frac{V_0}{\alpha_0}\ ,\quad
        s_{\ 4}^{(4)}=\frac{3}{2}\frac{V_0}{\alpha_0}\ ,\quad s_{\ 5}^{(4)}=\frac{11}{2}\frac{V_0}{\alpha_0}\ ,\\
        s_{\ n\geq 6}^{(4)}&=\left(-1\right)^{n}\frac{V_0}{\alpha_0}\left[\frac{21}{\left(n-2\right)!}-\frac{9}{\left(n-4\right)!}+\frac{1}{\left(n-6\right)!}\right]
    \end{split}
\end{equation}
We have:
\begin{equation}
    \begin{split}
       \frac{\alpha_0}{V_0}\sum_{n=0}^{\infty}s_{\ n}^{(4)}\phi^{n}\left(s\right)&=e^{-\phi}\left(\phi^6-9\phi^4+21\phi^2\right)
    \end{split}
\end{equation}

\begin{equation}
\begin{split}
        G_4\left(\phi\right)&= 2\sum_{n=1}^{\infty}ns_{\ n}^{(4)}\phi^{n-1}=2\de_\phi\sum_{n=0}^{\infty}s_{\ n}^{(4)}\phi^{n}\\
        &=-\frac{2V_0}{\alpha_0} \left(\phi^6-6\phi^5-9\phi^4+36\phi^3+21\phi^2-42\phi\right)e^{-\phi}
\end{split}
\end{equation}


==> Models/lc.tex <==
\subsection{Light-cone quantisation}
Due to its more direct connection to phenomenology, we will now focus on light-cone quantisation. Then, we will move on to constructing the space-time low energy spectrum of superstring theory. First of all, we introduce light-cone coordinates for bosonic degrees of freedom:
\begin{equation}
    X^{\pm}\equiv\frac{X^0\pm X^1}{\sqrt{2}}
\end{equation}
Now, we refer to the other $D-2$ transversal coordinates as $X^i$. After having defined similar components for the world-sheet fermions, we exploit our gauge freedom to fix:
\begin{equation}
    X^+=\frac{2\pi\alpha'}{l}p^+\tau\ ,\quad\psi^+=0\ .
\end{equation}
This way, both local reparametrisations and supersymmetry are exhausted. The open string light-cone Hamiltonian is
\begin{equation}
    H_{\text{open}}=
\end{equation}

==> Models/multiplescalars.tex <==
\subsubsection{Multiple scalar fields}
In the following derivation, we will generalise the previous result to a system to an arbitrarily large collection of scalar fields $\Phi=\left(\phi^1,\dots,\phi^N\right)$, where the rescaled dilaton, which plays a special role in defining the string frame action, is identified with $\phi^1$. For the sake of simplicity, we will now use $\mathbf{\Phi}_{\mathcal{M}}$ to refer to the collective moduli space of space-time configurations of such scalars, of which we can once more take the product with the generalised moduli space of geometries in order to obtain $\mathbf{\Gamma}_{\mathcal{M}}$. After having introduced the collection
\begin{equation}
    \Bar{n}\equiv\left(n^1,\dots,n^N\right)\in\N^N
\end{equation} 
of $N$ natural numbers, with $B_{\Bar{n}}$ being infinitely many couplings labelled by $\Bar{n}$, and an appropriately generalised family of constant, we can define the entropy functional:
\begin{equation}\label{genfunk}
\begin{split}
\mathcal{F}_{\Bar{\tau}}\left[g,\Phi\right]&=\int_{\mathcal{M}}\diff^{D}x\sqrt{-g}e^{-\phi^{1}}\Bigl[R_g+\sum_{i=1}^{\infty}\alpha_i\left(\nabla\phi^i\right)^2+\sum_{i=1}^{\infty}\gamma_i\nabla^2\phi^i\\
&\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad+\sum_{\Bar{n}\in\N^N}B_{\Bar{n}}\prod_{i=1}^N
    \left(\phi^{i}\right)^{n_i}\Bigr]\ .
\end{split}
\end{equation}
The notation $\Bar{\tau}$ collects the $\alpha_i$, the $\gamma_i$ and the $B_{\Bar{n}}$ constants, uniquely fixing \eqref{genfunk}. At this point, we assume field variations of the form:
\begin{equation}
    g_{\mu\nu}\rightarrow g_{\mu\nu}+v_{\mu\nu}\ ,\quad\phi^i\rightarrow\phi^i+h^i\ ,
\end{equation}
While performing volume preserving variations
\begin{equation}
    \delta\int_{\mathcal{M}}\diff^{D}x\sqrt{-g}e^{-\phi^{1}}=0
\end{equation}
fixes the usual condition 
\begin{equation}\label{volcostn}
    2h^1=g_{\mu\nu}v^{\mu\nu}=v
\end{equation}
on the rescaled dilaton variation, there is no a priori mechanism to impose similar conditions on the other scalars $\phi^2,\dots,\phi^N$. First of all, since we are always free to rescale the constants $\tau$ and the matter content of the theory, we can assume
\begin{equation}
    h\equiv h^2=\dots=h^N
\end{equation}
without loss of generality. The only further constraint might come from the general notion of moduli space distance introduced in \eqref{generalstdistance}. Since we will eventually apply our results to physical systems, it is reasonable to expect the scalar fields to have:
\begin{equation}\label{kinscal}
    \mathcal{L}_{\text{kin}}\sim-\frac{1}{2}\delta_{ij}\nabla^\mu\phi^i\nabla_\mu\phi^j\ .
\end{equation}
In general, \eqref{kinscal} can always be achievable by diagonalising the fields space coordinates. Plugging this simple structure into \eqref{generalstdistance} and also considering the variations of $g_{\mu\nu}$ and $\phi^1$, which are fixed in terms of $v_{\mu\nu}$, we would have the moduli space path length formula
\begin{equation}\label{lengthgen}
    \mathbf{L}\left[\Sigma\right]=\int_{s_0}^{s_1}\diff s\left|\ev{v^{\mu}{}_{\nu}v^{\nu}{}_{\mu}}+\frac{1}{8}\ev{v^2}+\frac{N-1}{2}\ev{h^{2}}\right|^{\frac{1}{2}}\ ,
\end{equation}
where $\Sigma\left(s\right)$ is a one-parameter curve in the generalised moduli space $\mathbf{\Gamma}_{\mathcal{M}}$, in which the geometry part was computed by taking the $\tau=0$ DeWitt metric. By imposing the generalised moduli space trajectory to extremise \eqref{lengthgen}, and thus be a geodesic, a constraint on $h$ in terms of $v_{\mu\nu}$ could be naturally achieved. Before doing so, we assume the simplest possible linear relation
\begin{equation}
    h\equiv\frac{\alpha}{2\sqrt{N-1}}v
\end{equation}
and reduce the length formula \eqref{lengthgen} to:
\begin{equation}\label{lengthgen2}
    \mathbf{L}\left[\Sigma\right]=\int_{s_0}^{s_1}\diff s\left|\ev{\text{Tr}\left[\left(G^{-1}\frac{\diff G}{\diff s}\right)^2\right]}+\frac{1+\alpha^2}{8}\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]^2}\right|^{\frac{1}{2}}\ ,
\end{equation}
Now, we will generalise the computation performed in \ref{subsub:metvar} and derive the geodesic equation associated to \eqref{lengthgen2}. Namely, we variate a path $\Sigma\equiv\left(G,\Phi\right)$ and impose the induced first order variation of the curve length to vanish. We obtain
\begin{equation}
    \delta\mathbf{L}\left[\Sigma\right]=\frac{1}{2}\int_{s_0}^{s_1}\diff s\left|\ev{\text{Tr}\left[\left(G^{-1}\frac{\diff G}{\diff s}\right)^2\right]}+\frac{1+\alpha^2}{8}\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]^2}\right|^{-\frac{1}{2}}\delta\mathcal{A}\ ,
\end{equation}
where we have defined the local variation
\begin{equation}
    \delta\mathcal{A}=\delta\mathcal{A}_{1}+\frac{1+\alpha^2}{8}\delta\mathcal{A}_{2}\ ,
\end{equation}
expressed as the sum of two terms:
\begin{equation}
    \delta\mathcal{A}_{1}\equiv\delta\ev{\text{Tr}\left[\left(G^{-1}\frac{\diff G}{\diff s}\right)^2\right]}\ ,\quad \delta\mathcal{A}_{2}\equiv\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]^2}\ .
\end{equation}
From the result expressed in \eqref{varfinmet}, we have that
\begin{equation}
    \begin{split}
        \delta\mathcal{A}_1&=\frac{1}{V_{\mathcal{M}}}\int_{\mathcal{M}} \text{vol}\left(G\right)\mathcal{B}_1\cdot\delta G\ ,
    \end{split}
\end{equation}
where we have defined:
\begin{equation}
    \begin{split}
        \mathcal{B}_1&\equiv G^{-1}\Biggl\{\frac{1}{2}\left(\text{Tr}\left[\left(G^{-1}\frac{\diff G}{\diff s}\right)^2\right]-\ev{\text{Tr}\left[\left(G^{-1}\frac{\diff G}{\diff s}\right)^2\right]}\right)G+2\frac{\diff G}{\diff s}G^{-1}\frac{\diff G}{\diff s}\\
        &\quad\quad\quad\quad-2\frac{\diff^2 G}{\diff s^2}+\left(\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]}-\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]\right)\frac{\diff G}{\diff s}\Biggr\}G^{-1}\ .
    \end{split}
\end{equation}
The second term, instead, requires us to perform an explicit computation. We obtain
\begin{equation}
    \begin{split}
        \delta\mathcal{A}_2&=\frac{1}{V_{\mathcal{M}}}\int_{\mathcal{M}} \text{vol}\left(G\right)\mathcal{B}_2\cdot\delta G\ ,
    \end{split}
\end{equation}
in which we have defined:
\begin{equation}
    \begin{split}
        \mathcal{B}_2&\equiv \frac{1}{2}\left(\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]^2-\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]^2}\right)G^{-1}+2\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]\frac{\diff G^{-1}}{\diff s}\\
        &\quad+\Biggl(\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]}-\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]\Biggr)\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]G^{-1}\\
        &\quad-2\Biggl(\text{Tr}\left[\frac{\diff G^{-1}}{\diff s}\frac{\diff G}{\diff s}\right]G^{-1}+\text{Tr}\left[G^{-1}\frac{\diff^2 G}{\diff s^2}\right]G^{-1}+\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]\frac{\diff G^{-1}}{\diff s}\Biggr)\ .
    \end{split}
\end{equation}
Therefore, imposing the overall variation
\begin{equation}
    \delta\mathcal{A}=\frac{1}{V_{\mathcal{M}}}\int_{\mathcal{M}} \text{vol}\left(G\right)\left(\mathcal{B}_{1}+C_\alpha\mathcal{B}_{2}\right)\cdot\delta G\ ,
\end{equation}
to vanish, with the constant $C_\alpha$ being defined as
\begin{equation}
    C_\alpha\equiv \frac{1+\alpha^2}{8}\ ,
\end{equation}
we are left with the geodesic equation:
\begin{equation}
    \begin{split}
        \frac{\diff^2 G}{\diff s^2}&=\frac{1}{4}\left(\text{Tr}\left[\left(G^{-1}\frac{\diff G}{\diff s}\right)^2\right]-\ev{\text{Tr}\left[\left(G^{-1}\frac{\diff G}{\diff s}\right)^2\right]}\right)G+\frac{\diff G}{\diff s}G^{-1}\frac{\diff G}{\diff s}\\
        &\quad+\frac{1}{2}\left(\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]}-\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]\right)\frac{\diff G}{\diff s}\\
        &\quad+\frac{C_\alpha}{4}\left(\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]^2-\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]^2}\right)G\\
        &\quad+\frac{C_\alpha}{2}\Biggl(\ev{\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]}-\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]\Biggr)\text{Tr}\left[G^{-1}\frac{\diff G}{\diff s}\right]G\\
        &\quad-C_\alpha\Biggl(\text{Tr}\left[\frac{\diff G^{-1}}{\diff s}\frac{\diff G}{\diff s}\right]G+\text{Tr}\left[G^{-1}\frac{\diff^2 G}{\diff s^2}\right]G\Biggr)\ .
    \end{split}
\end{equation}
Once more introducing $H^{\mu}{}_\nu$ as in \eqref{defH}, the above expression simplifies to:
\begin{equation}
    \begin{split}
        \frac{\diff H}{\diff s}+C_\alpha\text{Tr}\left[\frac{\diff H}{\diff s}\right]\mathbb{1}&=\frac{\mathbb{1}}{4}\left(\text{Tr}\left[H^2\right]-\ev{\text{Tr}\left[H^2\right]}\right)+\frac{1}{2}\left(\ev{\text{Tr}\left[H\right]}-\text{Tr}\left[H\right]\right)H\\
        &\quad-\frac{C_\alpha}{4}\left(\text{Tr}\left[H\right]^2-2\text{Tr}\left[H\right]\ev{\text{Tr}\left[H\right]}+\ev{\text{Tr}\left[H\right]^2}\right)\mathbb{1}\ .
    \end{split}
\end{equation}
%Derive geodesic equation in terms of alpha, compute variation and flow equations, plug everything back into the geodesic equation and see if some alpha satisfies it



\subsubsection{Multiple scalar fields}
Before analysing a family of relevant examples, we will generalise the previously developed discussion to an arbitrarily large collection of scalar fields $\Phi=\left(\phi^1,\dots,\phi^N\right)$, where the rescaled dilaton, which plays a special role in defining the string frame action, is identified with $\phi^1$. Therefore, we consider the $D$-dimensional Lorentzian action
\begin{equation}
    \tilde{S}\bigl[\tilde{g},F\bigr]\equiv\frac{1}{2\kappa^2_D}\int_{\mathcal{M}}\diff^Dx\sqrt{-\tilde{g}}\left[R_{\tilde{g}}-\frac{1}{2}\sum_{i=1}^N\left(\nabla f^i\right)^{2}-\sum_{\Bar{n}\in\N^N}G_{\Bar{n}}\prod_{i=1}^N
    \frac{\left(f^{i}\right)^{n_i}}{n_i!}\right]
\end{equation}
for the metric $\tilde{g}$ and the family of scalars $F\equiv\left(f^1,\dots,f^N\right)$, in which 
\begin{equation}
    \Bar{n}\equiv\left(n^1,\dots,n^N\right)\in\N^N
\end{equation} 
is a collection of $N$ natural numbers. At this point, we introduce the rescaled fields:
\begin{equation}
    \tilde{g}_{\mu\nu}\equiv e^{2\varphi}g_{\mu\nu},\quad f^i\equiv\sigma^i\phi^i\ .
\end{equation}
By doing so, the action becomes:
\begin{equation}
\begin{split}
        S\bigl[g,\Phi\bigr]&\equiv\frac{1}{2\kappa^2_D}\int_{\mathcal{M}}\diff^Dx\sqrt{-g}e^{\left(D-2\right)\varphi}\Biggl[R_g-(D-2)(D-1)\left(\nabla\varphi\right)^2\\
        &\quad-2(D-1)\nabla^2\varphi-\sum_{i=1}^N\frac{\left(\sigma^i\right)^{2}}{2}\left(\nabla \phi^i\right)^{2}-\sum_{\Bar{n}\in\N^N}G_{\Bar{n}}\prod_{i=1}^N
    \frac{\left(\phi^{i}\right)^{n_i}}{n_i!}\left(\sigma^{i}\right)^{n_i}\Biggr]\ .
\end{split}
\end{equation}
As was done in the previous derivation, we set:
\begin{equation}
    \varphi=\frac{1}{2-D}\phi^1\ ,\quad \sigma^1=\sqrt{\frac{2D-6}{D-2}}\ .
\end{equation}
By moreover taking $\sigma^j=1$ for each $j\geq2$, the expression for the action simplifies to:
\begin{equation}\label{msst2}
\begin{split}
        S\bigl[g,\Phi\bigr]&\equiv\frac{1}{2\kappa^2_D}\int_{\mathcal{M}}\diff^Dx\sqrt{-g}e^{-\phi^1}\Biggl\{R_g-2\left(\nabla\phi^1\right)^2+2\frac{D-1}{D-2}\nabla^2\phi^1\\
        &\quad\quad-\frac{1}{2}\sum_{j=2}^N\left(\nabla \phi^j\right)^{2}-\sum_{\Bar{n}\in\N^N}G_{\Bar{n}}\frac{\left(\phi^{1}\right)^{n_1}}{n_1!}\left(\frac{2D-6}{D-2}\right)^{n_1/2}\prod_{j=2}^N
    \frac{\left(\phi^{j}\right)^{n_j}}{n_j!}\Biggr\}\ .
\end{split}
\end{equation}
\newpage

==> Models/sclaaaa.tex <==
%show that GR alone is NOT enough! Except for cosmological constant and Einstein manifolds
By assuming the metric flow source to take the general form
\begin{equation}\label{singsource}
\begin{split}
         A_{\mu\nu}&\equiv -2R_{\mu\nu}+2\omega Rg_{\mu\nu}+ b\nabla_\mu\nabla_\nu\phi+g_{\mu\nu}d\Delta\phi\\
     &\quad+e\nabla_\mu\phi\nabla_\nu\phi+fg_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi\ ,
\end{split}
\end{equation}
the energy-momentum tensor flow source gets to be:
\be\label{osbssi}
\begin{split}
   2B_{\mu\nu}&=-2\nabla^\sigma\nabla_\nu R_{\mu\sigma}+2\left[1+\left(2-D\right)\omega\right]\nabla_\mu\nabla_\nu R+2\Delta R_{\mu\nu}-2\nabla_\mu\nabla^\sigma R_{\sigma\nu}\\
&\quad+\left[2\left(D-2\right)\omega-1 \right]g_{\mu\nu}\Delta R+2R_\mu{}^\sigma{}_\nu {}^\theta R_{\sigma\theta}+2RR_{\mu\nu}-2R_\mu{}^\sigma R_{\sigma\nu}\\
    &\quad-4\Lambda R_{\mu\nu}+2\left(C-R_{\sigma\theta}R^{\sigma\theta}+2\Lambda\omega R\right)g_{\mu\nu}+\Omega_{\mu\nu}\phi\\
    &\quad     +\Theta_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi+\Sigma_{\mu\nu}^{\sigma\theta}\nabla_\sigma\phi\nabla_\theta\phi\ .
\end{split}
\ee
Given the analysis performed in \cite{DeBiasio:2022omq}, we now want to find an entropy $\mathcal{F}$-functional
\begin{equation}\label{funk}
        \mathcal{F}_{\left(\alpha,\gamma\right)}\left(g,\phi\right)=\int\diff^{D}x\sqrt{g}e^{-\phi}\left[R+\alpha\left(\nabla\phi\right)^2+\gamma\Delta\phi\right]
\end{equation}
such that the flow sourced by \eqref{singsource} can be derived as its associated gradient flow equation for $g_{\mu\nu}$ and $\phi$. As discussed in the above-mentioned reference, we have that the volume-preserving gradient of \eqref{funk} gives:
\begin{equation}\label{geneqm}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}+2\left(1-\alpha+\gamma\right)\nabla_{\mu}\phi\nabla_{\nu}\phi-2\left(1+2\gamma\right)\nabla_{\nu}\nabla_{\mu}\phi+\\
        &+2\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\Delta\phi-2\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\left(\nabla\phi\right)^2\ ,
            \end{split}
\end{equation}
\begin{equation}\label{geneqs}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-R+\left[\left(1-\alpha\right)\left(1-D\right)+\gamma\left(1+\frac{D}{2}\right)\right]\left(\nabla\phi\right)^{2}+\\
        &-\left[1-D\left(1-\alpha\right)+\gamma\left(2+\frac{D}{2}\right)\right]\Delta\phi\ .
    \end{split}
\end{equation}
In order to match \eqref{singsource} with \eqref{geneqm}, we first have impose $\omega=0$. Furthermore, we must take $d=-f$ and select the following parameters:
\be 
\begin{split}
    b=-2\left(1+2\gamma\right)\ ,\quad d=-f=2\left(1-\alpha-\frac{\gamma}{2}\right)\ ,\quad e=2\left(1-\alpha+\gamma\right)\ .
\end{split}
\ee
The above equations directly imply:
\be 
\gamma=-\frac{b+2}{4}\ ,\quad \alpha=\frac{10-4d+b}{8}\ .
\ee
Hence, $e$ too gets fixed in terms of $b$ and $d$ as:
\be 
e=\frac{2+4d+b}{4}\ .
\ee 
Therefore, the restricted flow 
\be\label{mf}
\begin{split}
         \frac{\de g_{\mu\nu}}{\de\lambda}&\equiv -2R_{\mu\nu}+ b\nabla_\mu\nabla_\nu\phi+g_{\mu\nu}d\Delta\phi\\
         &\quad+\frac{2+4d+b}{4}\nabla_\mu\phi\nabla_\nu\phi-dg_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi
\end{split}
\ee
can be derived as the volume-preserving metric gradient flow of the entropy $\mathcal{F}$-functional:
\begin{equation}
        \mathcal{F}\left(g,\phi\right)=\int\diff^{D}x\sqrt{g}e^{-\phi}\left[R+\frac{10-4d+b}{8}\left(\nabla\phi\right)^2-\frac{b+2}{4}\Delta\phi\right]\ .
\end{equation}
If we wanted to also consider the associated scalar flow, we would have:
\begin{equation}\label{sf}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-R+\left[\frac{4d-b-2}{8}\left(1-D\right)-\frac{b+2}{4}\left(1+\frac{D}{2}\right)\right]\left(\nabla\phi\right)^{2}+\\
        &-\left[1-D\frac{4d-b-2}{8}-\frac{b+2}{4}\left(2+\frac{D}{2}\right)\right]\Delta\phi\\
        &\equiv-R+f_D\left(\nabla\phi\right)^{2}-g_D\Delta\phi\ .
    \end{split}
\end{equation}
What would assuming \eqref{mf} and \eqref{sf} imply for the energy-momentum tensor $T_{\mu\nu}$? In order to investigate such question, we start from
\be 
T_{\mu\nu}=\nabla_\mu\phi\nabla_\nu\phi-g_{\mu\nu}\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi+\frac{m^2}{2}\phi^2\right)\ ,
\ee 
where $m$ is the mass of the scalar field $\phi$. By taking the $\lambda$-derivative, we have:
\be
\begin{split}\label{indflowT}
    \frac{\de T_{\mu\nu}}{\de\lambda}\equiv E_{\mu\nu}&=-\nabla_\mu\phi\nabla_\nu R+f_D\nabla_\mu\phi\nabla_\nu\left(\nabla\phi\right)^{2}-g_D\nabla_\mu\phi\nabla_\nu\Delta\phi\\
    &\quad-\nabla_\nu\phi\nabla_\mu R+f_D\nabla_\nu\phi\nabla_\mu\left(\nabla\phi\right)^{2}-g_D\nabla_\nu\phi\nabla_\mu\Delta\phi\\
    &\quad-g_{\mu\nu}m^2\phi\left[-R+f_D\left(\nabla\phi\right)^{2}-g_D\Delta\phi\right]\\
    &\quad+g_{\mu\nu}\left[\nabla^\alpha\phi\nabla_\alpha R-f_D\nabla^\alpha\phi\nabla_\alpha\left(\nabla\phi\right)^{2}+g_D\nabla^\alpha\phi\nabla_\alpha\Delta\phi\right]\\
    &\quad+2R_{\mu\nu}\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi+\frac{m^2}{2}\phi^2\right)\\
    &\quad- b\nabla_\mu\nabla_\nu\phi\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi+\frac{m^2}{2}\phi^2\right)\\
    &\quad-g_{\mu\nu}d\Delta\phi\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi+\frac{m^2}{2}\phi^2\right)\\
    &\quad-\frac{2+4d+b}{4}\nabla_\mu\phi\nabla_\nu\phi\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi+\frac{m^2}{2}\phi^2\right)\\
         &\quad+dg_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi\left(\frac{1}{2}\nabla_\alpha\phi\nabla^\alpha\phi+\frac{m^2}{2}\phi^2\right)\ .
\end{split}
\ee
By selecting a specific flow for the metric tensor, we have thus obtained it as the gradient flow from an $\mathcal{F}$-entropy functional. Therefore, we managed to derived the associated scalar flow equation. Such a discussion directly implies an energy-momentum tensor flow sourced by \eqref{indflowT}. Conversely, by selecting the same flow for the metric tensor and imposing Einstein field equations to be on-shell along the flow, we have obtained an explicit expression \eqref{osbssi} for the required flow source of the energy-momentum tensor. Being the two different, we will apply the procedure described in section \ref{entropysection} and try to account for it by introducing extra matter fields in specific examples.
%compute it, compare it with B_munu: different. Either we assume phi not to follow that gradient flow or we allow new fields to enter the theory. How do you estimate their contribution? Take the B_munu-dT_munu\dl difference as the evolution of this extra source, set it equal to zero at the beginning and see how it behaves. Maybe, study only its trace (properly)!
%take a specific solution, like the one in which the cosmological constant is sourced by a scalar. Apply the machinery and see what happens
\subsubsection{An example in $D=2$}\label{specific}
We now focus on a specific and simple example, which will allow us to derive explicit and insightful results. First of all, we assume to work in $D=2$, with coordinates $\left(t,x\right)$. This way we can take a very simple ansatz for our static metric:
\be 
g_{\mu\nu}=\begin{pmatrix}
-g_1\left(x\right) & 0 \\
a & g_2\left(x\right)
\end{pmatrix}
\ee
Moreover, we assume the scalar field to be time-independent. The fact that we work in $D=2$ implies that:
\be 
R_{\mu\nu}=\frac{R}{2}g_{\mu\nu}\ .
\ee
It can be easily shown that all the above assumptions are conserved along the flow. On top of that, the non-trivial Christoffel symbols are:
\be 
\Gamma^t_{\ tx}=\Gamma^t_{\ xt}=\frac{g_1'}{2g_1}\ ,\quad\Gamma^x_{\ tt}=\frac{g_1'}{2g_2}\ ,\quad\Gamma^x_{\ xx}=\frac{g_2'}{2g_2}\ .
\ee 
We simply have $\nabla_\alpha\phi\nabla^\alpha\phi=\left(\phi'\right)^2/g_2$, where the prime-symbol stands for an $x$-derivative. In order to make our setting even simpler, we choose $d=b=0$ in the flow source $A_{\mu\nu}$, so that also $f=0$ and $e=1/2$, consistently with the derivation of our flow equations from the $\mathcal{F}$-functional. So, they reduce to:
\be\label{specflmet}
\begin{split}
         \frac{\de g_{\mu\nu}}{\de\lambda}&= -2R_{\mu\nu}+\frac{1}{2}\nabla_\mu\phi\nabla_\nu\phi\ ,
\end{split}
\ee
\begin{equation}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-R-\frac{3}{4}\left(\nabla\phi\right)^{2}\ .
    \end{split}
\end{equation}
Before writing them explicitly in terms of $g_1$ and $g_2$, we observe that:
\be 
R=\frac{g_2 \left[\left(g_1'\right)^2-2 g_1 g_1''\right]+g_1 g_1'g_2'}{2 g_1^2 g_2^2}
\ee 
Therefore, the three equations are:
\be
\begin{split}
         \frac{\de g_1}{\de\lambda}= -\frac{g_2 \left[\left(g_1'\right)^2-2 g_1 g_1''\right]+g_1 g_1'g_2'}{2 g_1 g_2^2}=-Rg_1\ ,
\end{split}
\ee
\be
\begin{split}
         \frac{\de g_2}{\de\lambda}=\equiv -\frac{g_2 \left[\left(g_1'\right)^2-2 g_1 g_1''\right]+g_1 g_1'g_2'}{2 g_1^2 g_2}+\frac{\left(\phi'\right)^2}{2}=-Rg_2+\frac{\left(\phi'\right)^2}{2}\ ,
\end{split}
\ee
\begin{equation}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-\frac{g_2 \left[\left(g_1'\right)^2-2 g_1 g_1''\right]+g_1 g_1'g_2'}{2 g_1^2 g_2^2}-\frac{3\left(\phi'\right)^2}{4g_2}=-R-\frac{3\left(\phi'\right)^2}{4g_2}\ .
    \end{split}
\end{equation}
Concerning the differential operators appearing in $B_{\mu\nu}$, we have $\Omega_{\mu\nu}=0$,
\be
\Theta_{\mu\nu}=\frac{1}{2}\left(g_{\mu\nu}\Delta-\nabla_\mu\nabla_\nu \right)\ ,
\ee
and, finally:
\be
\begin{split}
   \Sigma_{\mu\nu}^{\sigma\theta }&=\frac{1}{2}\Big[\left(R_\mu{}^\sigma+\nabla_\mu\nabla^\sigma \right)\delta_\nu^{\ \theta}+g_{\mu\nu}R^{\sigma\theta}-g_{\mu\nu}\nabla^\sigma\nabla^\theta -R_\mu{}^\sigma{}_\nu {}^\theta\\
&\quad+\left(2\Lambda-R-\Delta \right)\delta_{\mu}^{\ \sigma}\delta_{\nu}^{\ \theta}+\delta_{\mu}^{\ \sigma}\nabla^\theta\nabla_\nu\Big] \ .
\end{split}
\ee
Since we are in $D=2$, we simply set $\Lambda=C=0$. Thus, the expression \eqref{osbssi} for $B_{\mu\nu}$ therefore becomes:
\be
\begin{split}
   2B_{\mu\nu}=\Theta_{\mu\nu}\nabla_\alpha\phi\nabla^\alpha\phi+\Sigma_{\mu\nu}^{\sigma\theta}\nabla_\sigma\phi\nabla_\theta\phi\ .
\end{split}
\ee
Making the last terms explicit, we have:
\be
\begin{split}
    2B_{\mu\nu}&=\frac{1}{2}\Big[\delta_\nu^{\ \theta}\nabla_\mu\nabla^\sigma -g_{\mu\nu}\nabla^\sigma\nabla^\theta +\delta_{\mu}^{\ \sigma}\nabla^\theta\nabla_\nu\Big]\nabla_\sigma\phi\nabla_\theta\phi\\
&\quad-\frac{R}{4}\nabla_\mu\phi\nabla_\nu\phi+\frac{1}{2}\left(g_{\mu\nu}\Delta-\nabla_\mu\nabla_\nu \right)\nabla_\alpha\phi\nabla^\alpha\phi\\
&\quad-\Delta\left(\nabla_\mu\phi\nabla_\nu\phi\right)\ .
\end{split}
\ee
For the sake of simplicity, we can further assume the scalar field to be massless. Concerning $E_{\mu\nu}$, we are hence left with:
\be
\begin{split}
E_{\mu\nu}&=-\nabla_\mu\phi\nabla_\nu R-\nabla_\nu\phi\nabla_\mu R-\frac{3}{4}\nabla_\mu\phi\nabla_\nu\left(\nabla\phi\right)^{2}\\
    &\quad-\frac{3}{4}\nabla_\nu\phi\nabla_\mu\left(\nabla\phi\right)^{2}+\left(R_{\mu\nu}-\frac{1}{4}\nabla_\mu\phi\nabla_\nu\phi\right)\nabla_\alpha\phi\nabla^\alpha\phi\\
    &\quad+g_{\mu\nu}\left[\nabla^\alpha\phi\nabla_\alpha R+\frac{3}{4}\nabla^\alpha\phi\nabla_\alpha\left(\nabla\phi\right)^{2}\right]\ .
\end{split}
\ee
From such expressions, we can obtain $S_{\mu\nu}$ as $E_{\mu\nu}-B_{\mu\nu}$:
\be
\begin{split}\label{2ds}
    S_{\mu\nu}&=-\nabla_\mu\phi\nabla_\nu R-\nabla_\nu\phi\nabla_\mu R-\frac{3}{2}\nabla_\mu\phi\nabla^\alpha\phi\nabla_\nu\nabla_\alpha\phi\\
    &\quad-\frac{3}{2}\nabla_\nu\phi\nabla^\alpha\phi\nabla_\mu\nabla_\alpha\phi-\frac{1}{4}\nabla_\mu\phi\nabla_\nu\phi\nabla_\alpha\phi\nabla^\alpha\phi\\
    &\quad+g_{\mu\nu}\left[\nabla^\alpha\phi\nabla_\alpha R+\frac{3}{2}\nabla^\alpha\phi\nabla^\beta\phi\nabla_\alpha\nabla_\beta\phi\right]\\
&\quad+\frac{R}{4}\nabla_\mu\phi\nabla_\nu\phi-g_{\mu\nu}\left(\nabla^\beta\nabla_\beta\nabla_\alpha\phi\nabla^\alpha\phi+\nabla^\beta\nabla_\alpha\phi\nabla_\beta\nabla^\alpha\phi\right)\\
&\quad+\nabla^\alpha\nabla_\alpha\nabla_\mu\phi\nabla_\nu\phi+2\nabla^\alpha\nabla_\mu\phi\nabla_\alpha\nabla_\nu\phi\\
&\quad +\nabla_\mu\nabla_\nu\nabla_\alpha\phi\nabla^\alpha\phi+\nabla_\nu\nabla_\alpha\phi\nabla_\mu\nabla^\alpha\phi+\nabla_\mu\phi\nabla^\alpha\nabla_\alpha\nabla_\nu\phi\\
&\quad-\frac{1}{2}\nabla_\mu\phi\nabla^\theta\nabla_\nu\nabla_\theta\phi-\frac{1}{2}\nabla_\sigma\phi\nabla_\mu\nabla^\sigma\nabla_\nu\phi\\
&\quad -\frac{1}{2}\nabla^\theta\nabla_\nu\nabla_\mu\phi\nabla_\theta\phi-\frac{1}{2}\nabla_\nu\nabla_\mu\phi\nabla^\theta\nabla_\theta\phi-\frac{1}{2}\nabla^\theta\nabla_\mu\phi\nabla_\nu\nabla_\theta\phi\\
&\quad-\frac{1}{2}\nabla_\mu\nabla^\sigma\nabla_\sigma\phi\nabla_\nu\phi-\frac{1}{2}\nabla^\sigma\nabla_\sigma\phi\nabla_\mu\nabla_\nu\phi-\frac{1}{2}\nabla_\mu\nabla_\sigma\phi\nabla^\sigma\nabla_\nu\phi\\
&\quad+\frac{1}{2}g_{\mu\nu} \Big(\nabla^\sigma\nabla^\theta\nabla_\sigma\phi\nabla_\theta\phi+\nabla^\theta\nabla_\sigma\phi\nabla^\sigma\nabla_\theta\phi+\nabla^\sigma\nabla_\sigma\phi\nabla^\theta\nabla_\theta\phi\\
&\quad+\nabla_\sigma\phi\nabla^\sigma\nabla^\theta\nabla_\theta\phi\Big)\ .
\end{split}
\ee
Clearly, the expression \eqref{2ds} is still too complicated to be treated nicely. In order to simplify it, we refer to the explicit computations performed in \ref{app2d}. Such derivations allow us to observe that $\nabla_\alpha\nabla_\beta\phi=\nabla_\beta\nabla_\alpha\phi$. By exploiting such symmetry, we get:
\be
\begin{split}\label{2dssimp}
    S_{\mu\nu}&=-\nabla_\mu\phi\nabla_\nu R-\nabla_\nu\phi\nabla_\mu R-\frac{3}{2}\nabla_\mu\phi\nabla^\alpha\phi\nabla_\nu\nabla_\alpha\phi\\
    &\quad-\frac{3}{2}\nabla_\nu\phi\nabla^\alpha\phi\nabla_\mu\nabla_\alpha\phi-\frac{1}{4}\nabla_\mu\phi\nabla_\nu\phi\nabla_\alpha\phi\nabla^\alpha\phi\\
    &\quad+g_{\mu\nu}\left(\nabla^\alpha\phi\nabla_\alpha R+\frac{3}{2}\nabla^\alpha\phi\nabla^\beta\phi\nabla_\alpha\nabla_\beta\phi\right)\\
&\quad+\frac{R}{4}\nabla_\mu\phi\nabla_\nu\phi+\Delta\nabla_\mu\phi\nabla_\nu\phi+2\nabla^\alpha\nabla_\mu\phi\nabla_\alpha\nabla_\nu\phi\\
&\quad +\frac{1}{2}\nabla_\mu\nabla_\nu\nabla_\alpha\phi\nabla^\alpha\phi+\frac{1}{2}\nabla_\mu\phi\Delta\nabla_\nu\phi\\
&\quad -\frac{1}{2}\nabla^\theta\nabla_\nu\nabla_\mu\phi\nabla_\theta\phi-\nabla_\nu\nabla_\mu\phi\Delta\phi-\frac{1}{2}\nabla_\mu\Delta\phi\nabla_\nu\phi\\
&\quad+\frac{1}{2}g_{\mu\nu} \Big(\Delta\phi\Delta\phi+\nabla_\sigma\phi\nabla^\sigma\Delta\phi-\Delta\nabla^\theta\phi\nabla_\theta\phi-\nabla^\theta\nabla_\sigma\phi\nabla^\sigma\nabla_\theta\phi\Big)\ .
\end{split}
\ee
By assuming both $R$ and the initial scalar configuration to be constant, we have that such conditions are conserved along the whole flow. So, we get that $S_{\mu\nu}$ simplifies to:
\be
\begin{split}
    S_{\mu\nu}&=0\ .
\end{split}
\ee
At this point, we an explicitly solve the flow equations. We do so by taking the metric to be that of $2$-dimensional (Anti-)de Sitter spacetime
\be 
g_{1}=1-\frac{\kappa x^2}{2}\ ,\quad g_{2}=\frac{1}{g_1}
\ee 
for which we simply have:
\be 
R=\kappa\ .
\ee
From the flow equation \eqref{specflmet} and the assumption of having a spacetime-constant scalar field, we can derive the flow equation
\be 
\frac{\de R}{\de\lambda}=R^2
\ee
for the Ricci scalar $R$, which can be solved explicitly as:
\be 
R\left(\lambda\right)=\frac{R_0}{1-R_0\lambda}\ .
\ee
As is well-known from previous works \cite{Kehagias:2019akr,DeBiasio:2020xkv}, it is well known that:
\begin{itemize}
    \item When $R_0>0$, the evolution reaches a singularity at a finite flow time.
    \item When $R_0<0$, the evolution asymptotically flows to flat spacetime.
\end{itemize}
Thus, we have:
\be 
\kappa\left(\lambda\right)=\frac{\kappa_0}{1-\kappa_0\lambda}\ .
\ee 
Concerning the scalar flow equation
\be 
\frac{\de\phi}{\de\lambda}=-R\ ,
\ee 
we can solve it and get:
\be 
\phi\left(\lambda\right)=\phi_0+\int_0^\lambda\frac{\kappa_0}{\kappa_0\tau-1}\diff\tau=\phi_0+\log{\left(1-\kappa_0\lambda\right)}\ .
\ee 
Since $S_{\mu\nu}=0$, the $2$-dimensional example gives us no interesting behaviour. This is something that should have been expected. Indeed, general relativity is trivial in $D=2$ and the energy-momentum tensor for a constant scalar is null.

\subsubsection{An example in $D=3$}\label{specific2}
In the following discussion, we reproduce the analysis performed in \ref{specific} in the case in which $D=3$. In order to do so, we once more assume to work with an initial condition comprised of the metric of an Einstein manifold -more specifically, that of Anti de-Sitter spacetime in $D=3$- and a massless, scalar field with constant spacetime value $\phi_0$. 
By assuming, once more, $d=b=0$ in the flow equations, we are left with:
\be
\begin{split}
 \frac{\de g_{\mu\nu}}{\de\lambda}= -2R_{\mu\nu}+\frac{1}{2}\nabla_\mu\phi\nabla_\nu\phi\ ,\quad   
  \frac{\de\phi}{\de\lambda}=-R-\frac{3}{4}\left(\nabla\phi\right)^{2}\ .
\end{split}
\ee
Such equations conserve our assumptions on $g_{\mu\nu}$ and $\phi$, so that we get
\be
\frac{\de R}{\de\lambda}=\frac{2R^2}{3}\ ,\quad \frac{\de\phi}{\de\lambda}=-R\ ,
\ee
precisely as in \ref{specific}, except for a small deviation due to different dimensionality. 
By already removing the terms containing derivatives of $\phi$, plugging-in the expression of $R_{\mu\nu}$ in terms of $R$ and $g_{\mu\nu}$ and remembering Anti-de Sitter spacetime scalar curvature is linked to the cosmological constant $\Lambda$ by
\be \label{equal}
R=6\Lambda
\ee
the expression for $S_{\mu\nu}$ gets to be:
\be
\begin{split}
   S_{\mu\nu}&=\left(4\Lambda^2-C\right)g_{\mu\nu}\ .
\end{split}
\ee
Therefore, the flow equation for the emergent energy-momentum tensor $\hat{T}_{\mu\nu}$ is:
\be
\frac{\de\hat{T}_{\mu\nu}}{\de\lambda}=\left(4\Lambda^2-C\right)g_{\mu\nu}\ .
\ee
Plugging-in an ansatz of the form
\be
\hat{T}_{\mu\nu}=\frac{\hat{T}}{3}g_{\mu\nu}\ ,
\ee
our equation simply reduces to:
\be
\frac{\de\hat{T}}{\de\lambda}=3\left(4\Lambda^2-C\right)\ .
\ee
By imposing the initial condition $\hat{T}_{\mu\nu}=0$ and remembering that $C$ appeared as the flow-source for $\Lambda$, we can solve the above equation as:
\be
\hat{T}\left(\lambda\right)=12\int_0^\lambda\Lambda^2\left(\tau\right)\diff\tau-3\left[\Lambda\left(\lambda\right)-\Lambda_0\right]\ .
\ee
In the following, we will explore three natural behaviours for $\Lambda$. First of all, we can take it to be constant in the flow parameter. Hence, we have:
\be
\hat{T}\left(\lambda\right)=12\Lambda^2\lambda\ .
\ee
If we instead take $\Lambda$ to be exponentially dropping as
\be 
\Lambda\left(\lambda\right)=\Lambda_0e^{-\lambda}\ ,
\ee
we would get:
\be
\hat{T}\left(\lambda\right)=6\Lambda_0^2\left(1-e^{-2\lambda}\right)+3\Lambda_0\left(1-e^{-\lambda}\right)\ .
\ee
For large values of the flow parameter, we get:
\be 
\hat{T}\left(\lambda\right)=3\Lambda_0\left(2\Lambda_0+1\right)\ .
\ee 
By assuming $\Lambda_0=-1$, this would imply the behaviour depicted in figure \ref{fig}. 
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/onshell/That.png}
    \caption{Plot of $\hat{T}$ against the flow parameter $\lambda$.}
    \label{fig}
\end{figure}
Last, we must consider the case in which the \eqref{equal} is taken to hold for the whole flow. Thus, $S_{\mu\nu}=0$ and no extra energy-momentum tensor $\hat{T}_{\mu\nu}$ emerges. Generally speaking and assuming any emergent field to be a real scalar, an energy-momentum tensor satisfying $\hat{T}_{\mu\nu}=\frac{\hat{T}}{3}g_{\mu\nu}$ can only be achieved by imposing
\be
\hat{T}=-\sum_{k=1}^{M}\frac{3m_k^2}{2}\phi_k^2\ ,
\ee
where $\phi_k$ are $M$ emergent spacetime-constant fields, which we will from now on normalise to $\phi_k=\sqrt{2/3}$, and $m_k$ the corresponding mass scales. Thus, we get:
\be
\hat{T}=-\sum_{k=1}^{M}m_k^2\ .
\ee
Therefore, making such masses flow-dependent, we have:
\be 
\sum_{k=1}^{M}m_k^2\left(\lambda\right)=12\int_0^\lambda\Lambda^2\left(\tau\right)\diff\tau-3\left[\Lambda\left(\lambda\right)-\Lambda_0\right]\ .
\ee
Taking the masses to be distributed as 
\be
m_k=m\sqrt{n}
\ee
and assuming only a finite portion of them to enter the theory, we would get:
\be 
m^2\left(\lambda\right)=\frac{12}{C_M}\int_0^\lambda\Lambda^2\left(\tau\right)\diff\tau-\frac{3}{C_M}\left[\Lambda\left(\lambda\right)-\Lambda_0\right]\ ,
\ee
where the numerical constant is
\be
C_M\equiv \frac{M(M+1)}{2}
\ee
and depends on the number of extra fields we choose to include in the theory.
%\be
%\frac{1}{\alpha^2}=\frac{2\Lambda}{(1-D)(D-2)}
%\ee


==> Models/sextic.tex <==
\subsection{Scalar field with sextic potential}\label{potentialcase}
In the following discussion, we assume the scalar to be subject to a potential of the form
\be \label{6pot}
V\left(\phi\right)=\frac{V_0}{\alpha_0}\phi^2\left(\phi^4-9\phi^2+21\right)\ ,
\ee
with $\alpha_0=9-4\sqrt{2}$, so that the values of the potential minima of our interest are normalised to $V_0$, which is taken to be a positive parameter. The potential is shown in figure \ref{pottV}. The equations of motion for $\phi$ can be solved by taking the scalar to have the spacetime-constant value 
\be 
\phi_0\equiv\sqrt{3+\sqrt{2}}\ ,
\ee
corresponding to a minimum of the potential. This will serve as our initial flow configuration, together with an appropriate solution for the metric. It can be observed that the potential, with the above illustrated configuration for the scalar field, produces an effective cosmological constant term. Therefore, our initial metric will be that of $D$-dimensional de Sitter spacetime with scalar curvature:
\be 
R=\frac{2D}{D-2}V_0\ .
\ee
From this point on, we will take $V_0=1$ for the sake of simplicity. 
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/onshell/V.png}
    \caption{Plot of the behaviour of $V\left(\phi\right)$ around $\phi=0$, when $V_0=1$.}
    \label{pottV}
\end{figure}
From the expression \eqref{6pot} for the potential, the action self-interaction coupling constants can be read off as follows:
\be
g_2=\frac{42}{\alpha_0}\ ,\quad g_4=-\frac{9\cdot4!}{\alpha_0}\ ,\quad g_6=\frac{6!}{\alpha_0}\ .
\ee
%Which are the non-zero g_n terms?
%Derive the action-induced flow equations
%Solve them with this initial condition
%Derive the extra term required by on-shell flow




\newpage
Neglecting the diffeomorphism term, the flow equations
\begin{equation}\label{acteq}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}-g_{\mu\nu}\sum_{n=1}^{+\infty}ns_{\ n}^{(D)}\phi^{n-1}+4\frac{D-1}{D-2}\nabla_{\mu}\phi\nabla_{\nu}\phi\\
        &-2\frac{5D-6}{D-2}\nabla_{\nu}\nabla_{\mu}\phi-2\frac{D-1}{D-2}g_{\mu\nu}\nabla^{2}\phi+2\frac{D-1}{D-2}g_{\mu\nu}\left(\nabla \phi\right)^2\ ,\\
        \frac{\de \phi}{\de\lambda}=&-R-\frac{D}{2}\sum_{n=1}^{+\infty}ns_{\ n}^{(D)} \phi^{n-1}+\frac{\left(D-1\right)\left(D+2\right)}{D-2}\left(\nabla \phi\right)^{2}\\
        &-\frac{D^{2}+4D-6}{D-2}\nabla^{2} \phi\ ,
    \end{split}
\end{equation}
where the $s_{\ k}^{(D)}$ parameters have been defined as:
\be 
    s_{\ k}^{(D)}\equiv\sum_{n=0}^{k}\frac{g_{n}}{\left(k-n\right)!n!}\left(\frac{2}{2-D}\right)^{k-n}\left(\frac{4D-6}{D-2}\right)^{n/2}\ .
\ee
For the specific case of the potential
\be
V\left(\phi\right)=\frac{1}{\alpha_0}\phi^2\left(\phi^4-9\phi^2+21\right)\ ,
\ee
with $\alpha_0=9-4\sqrt{2}$, we have:

Hence, the $s_{\ k}^{(D)}$ parameters are:
\be
\begin{split}
    s_{\ 0}^{(D)}&=s_{\ 1}^{(D)}=0\ ,\quad s_{\ 2}^{(D)}=\frac{42}{\alpha_0}\cdot\frac{2D-3}{D-2}\ ,\quad
    s_{\ 3}^{(D)}=-\frac{84}{\alpha_0}\cdot\frac{2D-3}{\left(D-2\right)^2}\ ,\\ s_{\ 4}^{(D)}&=-\frac{12}{\alpha_0}\cdot\frac{2D-3}{\left(D-2\right)^3}\left(6D^2-21D+11\right)\ ,\\
    s_{\ 5}^{(D)}&=\frac{8}{\alpha_0}\cdot\frac{2D-3}{(D-2)^4}\left(18D^2-27D-36D+47\right)\ ,\\
    s_{\ k\geq 6}^{(D)}&=\frac{(-1)^k2^{k-3}}{\left(k-6\right)!\alpha_0}\cdot\frac{2D-3}{(D-2)^{k-3}}\Bigg[
    \frac{84\left(k-6\right)!}{\left(k-2\right)!(D-2)^2}\\
    &\quad-\frac{9\left(k-6\right)!\left(4D-6\right)}{\left(k-4\right)!(D-2)}+\left(2D-3\right)^{2}\Bigg]\ .
\end{split}
\ee
Defining the simpler parameters
\be 
g_{\ k}^{(D)}\equiv\alpha_0s_{\ k}^{(D)}
\ee
and taking $D=4$ for the sake of simplicity, we get:
\be
\begin{split}
    g_{\ 0}^{(4)}&=g_{\ 1}^{(4)}=0\ ,\quad g_{\ 2}^{(4)}=105\ ,\quad
    g_{\ 3}^{(4)}=-105\ ,\\ g_{\ 4}^{(4)}&=-\frac{345}{2}\ ,\quad g_{\ 5}^{(4)}=\frac{415}{2}\ ,\\
g_{\ k\geq6}^{(4)}&=(-1)^k\Bigg[
    \frac{105}{\left(k-2\right)!}-\frac{225}{\left(k-4\right)!}+\frac{125}{\left(k-6\right)!}\Bigg]\ .
\end{split}
\ee
The explicit $k$-behaviour of such factors is shown in figure \ref{ddott}.
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Figures/onshell/dotspl.png}
    \caption{Plot of $g_{\ k}^{(4)}$ for different values of $k$, at $D=4$. Clearly, the coefficients drop to zero in an extremely quick way.}
    \label{ddott}
\end{figure}
At this point, we must compute the value of the function:
\be 
F\left(\phi\right)\equiv \sum_{n=1}^{+\infty}ns_{\ n}^{(4)} \phi^{n-1}\ .
\ee
Therefore, we have:
\be 
\begin{split}
    \alpha_0F\left(\phi\right)&=210\phi-315\phi^2-690\phi^3+\frac{2075}{2}\phi^4\\
    &\quad+\sum_{k=6}^{+\infty}k(-1)^k\Bigg[
    \frac{105}{\left(k-2\right)!}-\frac{225}{\left(k-4\right)!}+\frac{125}{\left(k-6\right)!}\Bigg]\phi^{k-1}\\
    &=210\phi-315\phi^2-690\phi^3+\frac{2075}{2}\phi^4\\
    &\quad+105\phi\left[2\sum_{n=4}^{+\infty}\frac{(-\phi)^n}{n!}-\phi\sum_{l=3}^{+\infty}
    \frac{(-\phi)^l}{l!}\right]\\
    &\quad-225\phi^3\left[4\sum_{n=2}^{+\infty}\frac{(-\phi)^n}{n!}-\phi\sum_{l=1}^{+\infty}\frac{(-\phi)^{l}}{l!}\right]\\
    &\quad+125\phi^5\left[6\sum_{n=0}^{+\infty}\frac{(-\phi)^n}{n!}-\phi\sum_{l=0}^{+\infty}\frac{(-\phi)^l}{l!}\right]\\
    &=210\phi-315\phi^2-690\phi^3+\frac{2075}{2}\phi^4\\
    &\quad+105\phi\left[\left(2-\phi\right)\left(e^{-\phi}-1+\phi-\frac{\phi^2}{2}\right)+\frac{\phi^3}{3}\right]\\
    &\quad-225\phi^3\left[\left(4-\phi\right)\left(e^{-\phi}-1\right)+4\phi\right]+125\phi^5\left(6-\phi \right)e^{-\phi}\\
   &=5\left[42\phi-21\phi^2-220\phi^3+55\phi^4+150\phi^5-25\phi^6\right]e^{-\phi}\ .
\end{split}
\ee
In the end, we get:
\be
F\left(\phi\right)=\frac{5}{\alpha_0}\left[42\phi-21\phi^2-220\phi^3+55\phi^4+150\phi^5-25\phi^6\right]e^{-\phi}\ .
\ee
The plot of such a function is given in figure \ref{Fpl}. Given that
we start with constant curvature and scalar field, it can be shown that the flow equations \eqref{acteq} preserve such conditions. Thus, they reduce to:
\begin{equation}
    \begin{split}
        \frac{\de R}{\de\lambda}=&-\frac{R}{2}\left[R+2F\left(\phi\right)\right]\ ,\\
        \frac{\de \phi}{\de\lambda}=&-\left[R+2F\left(\phi\right)\right]\ .
    \end{split}
\end{equation}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/onshell/FFF.png}
    \caption{Plot of F against $\phi$, in which the exponential suppression can be observed.}
    \label{Fpl}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/onshell/Rphi.png}
    \caption{Flow behaviour for $R$ and $\phi$.}
    \label{fflo}
\end{figure}
Given the $D=4$ initial conditions
\be 
\phi_0\equiv\sqrt{3+\sqrt{2}}\ ,\quad R_0=4\ ,
\ee
the flow can be straightforwardly solved numerically, as shown in figure \ref{fflo}. More generally, figure \ref{vec} shows the vector fields tangent to the flow, in the $\left(R,\phi\right)$ space.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/onshell/Vector.png}
    \caption{Plot of the vector field tangent to the flow, in the $\left(R,\phi\right)$ space.}
    \label{vec}
\end{figure}
As in the previous derivation, we have $B_{\mu\nu}=0$ and
\be 
S_{\mu\nu}=C_0g_{\mu\nu}\ ,
\ee
with:
\be
\begin{split}
   C_0&=-\frac{1}{\alpha_0 }\left(\phi^6+12\phi^5-9\phi^4-72\phi^3+21\phi^2+84\phi\right)\left[\frac{R}{2}+F\left(\phi\right)\right]\ .
\end{split}
\ee
In figure \ref{ssoss}, the explicit flow behaviour of $C_0$ is shown. There we can observe that it goes to positive values, then to slightly negative ones and finally tends to zero. 
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/onshell/Czero.png}
    \caption{Plot of $C_0$ against the flow parameter $\lambda$.}
    \label{ssoss}
\end{figure}
By introducing an extra energy-momentum tensor with the simple diagonal form 
\be 
\hat{T}_{\mu\nu}=\Omega g_{\mu\nu}\ ,
\ee
we have that $\Omega$ follows the simple flow equation:
\begin{equation}
    \frac{\de\Omega}{\de\lambda}=C_0\ .
\end{equation}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/onshell/aOmega.png}
    \caption{Plot of $\Omega$ against the flow parameter $\lambda$.}
    \label{sssoss}
\end{figure}
In figure \ref{sssoss}, it can be observed that $\Omega$ approaches the constant asymptotic value $\Omega_\infty\sim 1.52$. 











==> Models/tt.tex <==
\paragraph{Traceless deformations}
In this example, we consider traceless metric variations
\begin{equation}
    T_{\mu\nu}\left(s\right)=g_{\mu\nu}+t_{\mu\nu}\left(s\right)\ ,
\end{equation}
where we have imposed $s\in\left[s_0,s_1\right]$, $t_{\mu\nu}\left(s_0\right)=0$ and:
\begin{equation}
    T^{\mu\nu}\left(s\right)t_{\mu\nu}\left(s\right)=t^{\mu}{}_{\mu}\left(s\right)=0\ .
\end{equation}
Under such assumptions, the curve length formula \eqref{ttdistance} simplifies to:
\begin{equation}
        \mathbf{L}_{\tau}\left[T\right]=\int_{s_0}^{s_1}\diff s\left[\frac{1}{V_{\mathcal{M}}}\int_{\mathcal{M}}\diff^Dx\sqrt{-G}\left(G^{\mu\nu}G^{\alpha\beta}-\tau G^{\mu\alpha}G^{\nu\beta}\right)\frac{\diff G_{\mu\alpha}}{\diff s}\frac{\diff G_{\nu\beta}}{\diff s}\right]^{\frac{1}{2}}\ .
\end{equation}
%MUST BE COMPLETED

==> Sections/Appendices/KKgeneral.tex <==
In the following discussion, we will start from a $\left(d+1\right)$-dimensional general relativistic gravitational theory, defined on a Lorentzian manifold $\mathcal{M}$ parametrised by coordinates $x^M$, with the useful notation choice:
\begin{equation}
    x=\left(x^0,\dots,x^{d-1},\lambda\right)\ .
\end{equation}
For the sake of simplicity, we refer to the first $d$ coordinates with the notation $x^\mu$. The action for the $\left(d+1\right)$-dimensional metric tensor $G_{MN}$ is:
\begin{equation}
    S=\frac{1}{\kappa_{d+1}^2}\int_{\mathcal{M}}\diff^{d}x\diff\lambda\sqrt{-G}R_G\ .
\end{equation}
Now, we introduce the metric decomposition
\begin{equation}
    G_{MN} \equiv \begin{pmatrix}
 g_{\mu\nu} & 0\\
 0 & \varphi\end{pmatrix}\ ,
\end{equation}
in which we have used a $d$-dimensional Lorentzian metric $g_{\mu\nu}$ and a scalar $\varphi$ on the $\left(d+1\right)$-dimensional space-time. This is by no means a general ansatz, since we have set the vector component of the metric to zero, but will be enough for our derivation. In particular, we have assumed
\begin{equation}
    \mathcal{M}=\mathcal{N}\times\mathcal{I}\ ,
\end{equation}
in which $\mathcal{N}$ is the $d$-dimensional manifold parametrised by $x^\mu$ and $\mathcal{I}$ is the $1$-dimensional manifold on which $\lambda$ is defined. The inverse metric is:
\begin{equation}
    G^{MN} \equiv \begin{pmatrix}
 g^{\mu\nu} & 0 \\
 0 &  1/\varphi
\end{pmatrix}.
\end{equation}
Now, we have to write down the decomposed form of the metric determinant $G$ and the Ricci scalar $R_G$. The Christoffel symbols $\Gamma^{M}_{NP}$ decompose as follows:
\begin{equation}
    \begin{split}
        2\Gamma^{N}_{PQ}&=G^{N\mu}\left(G_{P\mu,Q}+G_{Q\mu,P}-G_{PQ,\mu}\right)\\
        &\quad+G^{Nd}\left(G_{Pd,Q}+G_{Qd,P}-G_{PQ,d}\right)\ .
    \end{split}
\end{equation}
Focusing on the various specific indices choices, we have:
\begin{equation}
    \begin{split}
        2\Gamma^{\nu}_{\alpha\beta}&=g^{\nu\mu}\left(g_{\alpha\mu,\beta}+g_{\alpha\mu,\beta}-g_{\alpha\beta,\mu}\right)\ ,\quad 
        2\Gamma^{d}_{dd}=\de_d\log{\varphi}\ ,\quad 2\Gamma^{\nu}_{dd}=-\de^\nu\varphi\ ,\\
        2\Gamma^{d}_{\alpha\beta}&=-\varphi^{-1}g_{\alpha\beta,d}\ ,\quad 
        2\Gamma^{\nu}_{\alpha d}=g^{\nu\mu}g_{\alpha\mu,d}\ ,\quad 2\Gamma^{d}_{d\mu}=\de_\mu\log{\varphi}\ .
    \end{split}
\end{equation}
Concerning the Ricci tensor, we get:
\begin{equation}
    R_{MN}= \partial_P\Gamma_{MN}^P - \partial_N\Gamma_{PM}^P + \Gamma_{PQ}^P\Gamma_{MN}^Q - \Gamma_{MQ}^P\Gamma_{PN}^Q\ .
\end{equation}
Referring to the Ricci tensor and covariant derivative on $\mathcal{N}$ as $\Tilde{R}_{\mu\nu}$ and $\tilde{\nabla}$, we obtain:
\begin{equation}
    \begin{split}
        2R_{\mu\nu}&=2\Tilde{R}_{\mu\nu}- \Tilde{\nabla}_\mu\Tilde{\nabla}_\nu\log{\varphi}
 +\frac{1}{\varphi}g_{\mu\nu,d}\partial_d\log{\varphi}
-\frac{1}{2\varphi}g_{\mu\nu,d}\left(\de_d\log{\varphi}+g^{\alpha\rho}g_{\alpha\rho,d}\right)\\
        &\quad+\frac{1}{\varphi} g^{\alpha\rho}g_{\mu\alpha,d} g_{\nu\rho,d}-\frac{1}{\varphi}\de_dg_{\alpha\beta,d}- \frac{1}{2}\de_\mu\log{\varphi}\de_\nu\log{\varphi}\ ,\\
        2R_{dd}&=-\Tilde{\nabla}^2\varphi+\frac{1}{2\varphi}\left(\de_\alpha\varphi\de^\alpha\varphi+g^{\alpha\mu}g_{\alpha\mu,d}\de_d\varphi\right)\\
        &\quad- \partial_d \left(g^{\alpha\mu}g_{\alpha\mu,d}\right)- \frac{1}{2}g^{\alpha\nu}g^{\beta\mu}g_{\beta\nu,d}g_{\alpha\mu,d}\ ,\\
        2R_{d\nu}&=\partial_\alpha\left(g^{\alpha\mu}g_{\nu\mu,d}\right)- \partial_\nu \left(g^{\alpha\mu}g_{\alpha\mu,d}\right)+ \Gamma_{\alpha\beta}^\alpha g^{\beta\mu}g_{\nu\mu,d}- \Gamma_{\alpha\nu}^\beta g^{\alpha\mu}g_{\beta\mu,d}\\
        &\quad+ \frac{1}{2}g^{\alpha\mu}g_{\alpha\mu,d}\de_\nu\log{\varphi}-\frac{1}{2}\de^\alpha\log{\varphi}g_{\alpha\nu,d}\ .
    \end{split}
\end{equation}
Now, we assume the $d$-dimensional metric $g_{\mu\nu}$ to evolve according to Ricci flow along $\lambda$:
\begin{equation}
    g_{\mu\nu,d}=-2\Tilde{R}_{\mu\nu}\ .
\end{equation}
Hence, we get:
\begin{equation}
    \begin{split}
        2R_{\mu\nu}&=2\Tilde{R}_{\mu\nu}- \Tilde{\nabla}_\mu\Tilde{\nabla}_\nu\log{\varphi}
 -\frac{2}{\varphi}\Tilde{R}_{\mu\nu}\partial_d\log{\varphi}
+\frac{1}{\varphi}\Tilde{R}_{\mu\nu}\left(\de_d\log{\varphi}-2\Tilde{R}\right)\\
        &\quad+\frac{4}{\varphi} g^{\alpha\rho}\Tilde{R}_{\mu\alpha} \Tilde{R}_{\nu\rho}+\frac{2}{\varphi}\de_d\Tilde{R}_{\mu\nu}- \frac{1}{2}\de_\mu\log{\varphi}\de_\nu\log{\varphi}\ ,\\
        2R_{dd}&=-\Tilde{\nabla}^2\varphi+\frac{1}{2\varphi}\left(\de_\alpha\varphi\de^\alpha\varphi-2\Tilde{R}\de_d\varphi\right)+2 \partial_d \Tilde{R}-2\Tilde{R}^{\alpha\mu}\Tilde{R}_{\alpha\mu}\ ,\\
        2R_{d\nu}&=2 \partial_\nu\Tilde{R}-2\nabla_\alpha\Tilde{R}^{\alpha}{}_\nu-\Tilde{R}\de_\nu\log{\varphi}+\Tilde{R}_{\nu\alpha}\de^\alpha\log{\varphi}\ .
    \end{split}
\end{equation}
The Ricci scalar is simply given by:
\begin{equation}
    \begin{split}
        2R&=2g^{\mu\nu}R_{\mu\nu}+2\varphi^{-1}R_{dd}\\
        &=2\Tilde{R}- \Tilde{\nabla}^2\log{\varphi}
-\frac{1}{\varphi}\Tilde{R}\left(\de_d\log{\varphi}+2\Tilde{R}\right)\\
        &\quad+\frac{2}{\varphi} \Tilde{R}^{\mu\alpha} \Tilde{R}_{\mu\alpha}+\frac{2}{\varphi}g^{\mu\nu}\de_d\Tilde{R}_{\mu\nu}- \frac{1}{2}\de^\mu\log{\varphi}\de_\mu\log{\varphi}\\
        &\quad-\varphi^{-1}\Tilde{\nabla}^2\varphi+\frac{1}{2\varphi^2}\left(\de_\alpha\varphi\de^\alpha\varphi-2\Tilde{R}\de_d\varphi\right)+2 \varphi^{-1}\partial_d \Tilde{R}\ .
    \end{split}
\end{equation}
If we assume $\varphi=1$, we obtain:
\begin{equation}
    \begin{split}
        R_{\mu\nu}&=\Tilde{R}_{\mu\nu}-\Tilde{R}\Tilde{R}_{\mu\nu}+2g^{\alpha\rho}\Tilde{R}_{\mu\alpha} \Tilde{R}_{\nu\rho}+\de_d\Tilde{R}_{\mu\nu}\ ,\\
        R_{dd}&= \partial_d \Tilde{R}-\Tilde{R}^{\alpha\mu}\Tilde{R}_{\alpha\mu}\ ,\\
        R_{d\nu}&=2 \partial_\nu\Tilde{R}-\nabla_\alpha\Tilde{R}^{\alpha}{}_\nu\ ,\\
        R&=\Tilde{R}-\Tilde{R}^2+\Tilde{R}^{\mu\alpha} \Tilde{R}_{\mu\alpha}+g^{\mu\nu}\de_d\Tilde{R}_{\mu\nu}+\partial_d \Tilde{R}\ .
    \end{split}
\end{equation}
Starting from the $\left(d+1\right)$-dimensional Einstein field equations
\begin{equation}
    2R_{MN}=G_{MN}R\ ,
\end{equation}
we obtain the various components:
\begin{equation}
    \begin{split}
        \Tilde{R}_{\mu\nu}-\Tilde{R}\Tilde{R}_{\mu\nu}+2g^{\alpha\rho}\Tilde{R}_{\mu\alpha} \Tilde{R}_{\nu\rho}+\de_d\Tilde{R}_{\mu\nu}&=\frac{1}{2}g_{\mu\nu}\left(\Tilde{R}-\Tilde{R}^2+\Tilde{R}^{\mu\alpha} \Tilde{R}_{\mu\alpha}+g^{\mu\nu}\de_d\Tilde{R}_{\mu\nu}+\partial_d \Tilde{R}\right)\\
        \partial_d \Tilde{R}-\Tilde{R}^{\alpha\mu}\Tilde{R}_{\alpha\mu}&=\frac{1}{2}\left(\Tilde{R}-\Tilde{R}^2+\Tilde{R}^{\mu\alpha} \Tilde{R}_{\mu\alpha}+g^{\mu\nu}\de_d\Tilde{R}_{\mu\nu}+\partial_d \Tilde{R}\right) \\
        2 \partial_\nu\Tilde{R}-\nabla_\alpha\Tilde{R}^{\alpha}{}_\nu&=0\ .
    \end{split}
\end{equation}
The last one is simply the Bianchi identity in $d$ dimensions. Combining the first and the second one, we get:
\begin{equation}
    \Tilde{R}_{\mu\nu}-\Tilde{R}\Tilde{R}_{\mu\nu}+2g^{\alpha\rho}\Tilde{R}_{\mu\alpha} \Tilde{R}_{\nu\rho}+\de_d\Tilde{R}_{\mu\nu}=g_{\mu\nu}\left(\partial_d \Tilde{R}-\Tilde{R}^{\alpha\mu}\Tilde{R}_{\alpha\mu}\right)
\end{equation}
Contracting with $g^{\mu\nu}$:
\begin{equation}
    \Tilde{R}-\Tilde{R}^2+(2+d)\Tilde{R}^{\mu\nu} \Tilde{R}_{\mu\nu}+g^{\mu\nu}\de_d\Tilde{R}_{\mu\nu}=d\partial_d \Tilde{R}
\end{equation}

==> Sections/On-Shellflow/realonshell.tex <==
\label{gfaa}
Let's consider a $D$-dimensional Riemannian manifold $\mathcal{M}$, over which a metric tensor $g_{\mu\nu}$ and a scalar $\varphi$ are defined. Furthermore, let their dynamics be governed by the Euclidean action:
\begin{equation}
    \mathcal{S}\left[g,\varphi\right]\equiv\frac{1}{2\kappa}\int\diff^Dx\sqrt{g}R+\int\diff^Dx\sqrt{g}\left(\frac{1}{2}\nabla^{\mu}\varphi\nabla_{\mu}\varphi+\beta_{n}\varphi^{n}+\beta_{m}\varphi^{m}\right)\ .
\end{equation}
The energy-momentum tensor associated to the matter part $\mathcal{S}_m\left[g,\varphi\right]$ of the action can be obtained as:
\begin{equation}
    T_{\mu\nu}\equiv\frac{1}{\sqrt{g}}\frac{\delta\mathcal{S}_m}{\delta g^{\mu\nu}}=\frac{1}{2}\nabla_{\mu}\varphi\nabla_{\nu}\varphi-\frac{1}{2}g_{\mu\nu}\left(\nabla_{\alpha}\varphi\nabla^{\alpha}\varphi+\beta_{n}\varphi^{n}+\beta_{m}\varphi^{m}\right)\ .
\end{equation}
Thus, the equations of motion associated to $\mathcal{S}\left[g,\varphi\right]$ are:
\begin{equation}
        R_{\mu\nu}-\frac{1}{2}g_{\mu\nu}R=\kappa T_{\mu\nu}\ ,\quad \nabla^2\varphi=n\beta_{n}\varphi^{n-1}+m\beta_{m}\varphi^{m-1}\ .
\end{equation}
Now, we consider the simplest possible non-trivial ansatz we can think of. Namely, we assume the geometry to be that of an \textit{Einstein manifold} and the scalar field to be \textit{constant}. Indeed, these assumptions can be phrased as:
\begin{equation}
    R_{\mu\nu}=\frac{R}{D}g_{\mu\nu}\ ,\quad \nabla_{\mu}\varphi=0\ .
\end{equation}
Plugging such conditions into the equations of motion, we are simply left with:
\begin{equation}
\begin{split}
R=&\frac{D\kappa}{D-2}\left(\beta_{n}\varphi^{n}+\beta_{m}\varphi^{m}\right)\ ,\\
    \varphi=&\left(-\frac{m\beta_m}{n\beta_n}\right)^{\frac{1}{n-m}}\ . 
\end{split}
\end{equation}
By inserting the expression for $\varphi$ into $R$, we get:
\begin{equation}
    R=\frac{D\kappa}{D-2}\left[\beta_{n}\left(-\frac{m\beta_m}{n\beta_n}\right)^{\frac{n}{n-m}}+\beta_{m}\left(-\frac{m\beta_m}{n\beta_n}\right)^{\frac{m}{n-m}}\right]\ .
\end{equation}
The \textit{most general} way in which we can understand the reduced moduli space we get when considering Einstein manifolds with a space-time constant scalar is that of a $6$-dimensional object, parametrised by $\left(D,\kappa,n,m,\beta_{m},\beta_n\right)$. Now, we want to further reduce it by fixing some of the quantities listed above. We take $\kappa=1/2$ and
\begin{equation}
    \beta_n=\frac{\lambda}{n!}\ ,\quad \beta_m=\frac{\lambda}{m!}\ .
\end{equation}
Now, the only free parameters are $\left(D,n,m,\lambda\right)$. Since we are working with a real scalar field, we must take $n>2$ and $m>2$ so that:
\begin{equation}
    \varphi=\left[-\frac{\left(n-1\right)!}{\left(m-1\right)!}\right]^{\frac{1}{n-m}}\in\R\ .
\end{equation}
This can be achieved by requiring:
\begin{equation}
    \frac{1}{n-m}\equiv k\in\Z\ .
\end{equation}
In order for $n$ to be integer, we must have
\begin{equation}
    n=m\pm1\ ,
\end{equation}
where $k=\pm 1$ is an integer parameter classifying alternative theories.
Since the $k=\pm 1$ theories are equivalent under exchange of $n$ and $m$, we can take, without loss of generality, $n=m+1$. Hence, we get
\begin{equation}
\begin{split}
\varphi&=-m\ ,\\
    R&=\frac{D}{D-2}\frac{\lambda}{2}\frac{\left(-m\right)^m}{\left(m+1\right)!}\ .
\end{split}
\end{equation}
In the above expressions, $m$ and $D$ are positive natural numbers, with $D>2$ for gravity to be dynamical, and $\lambda$ is a positive real number. One can straightforwardly observe that the moduli of $\varphi$ and $R$ grow with $m$, where $R$ is \textit{positive} for \textit{even} $m$ and \textit{negative} for \textit{odd} $m$. Namely, odd and even $m$ realise Anti de Sitter and de Sitter space-time, respectively. Given our assumptions on the theory parameters, the action reduces to:
\begin{equation}\label{reda}
    \mathcal{S}\left[g,\varphi\right]\equiv\int\diff^Dx\sqrt{g}\left[R+\frac{1}{2}\left(\nabla\varphi\right)^2+\frac{\lambda\varphi^{m}}{m!}+\frac{\lambda\varphi^{m+1}}{\left(m+1\right)!}\right]\ .
\end{equation}
This can be directly connected to the derivation of flow equations from an action performed in \eqref{gfa}. Namely, we can use \eqref{reda} to read off the flow equations
\begin{equation}\label{acteq}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}-g_{\mu\nu}\sum_{n=1}^{+\infty}ns_{\ n}^{(D)}\varphi^{n-1}+4\frac{D-1}{D-2}\nabla_{\mu}\varphi\nabla_{\nu}\varphi-2\frac{5D-6}{D-2}\nabla_{\nu}\nabla_{\mu}\varphi+\\
        &-2\frac{D-1}{D-2}g_{\mu\nu}\nabla^{2}\varphi+2\frac{D-1}{D-2}g_{\mu\nu}\left(\nabla \varphi\right)^2+\mathcal{L}_{\xi}g_{\mu\nu}\ ,\\
        \frac{\de \varphi}{\de\lambda}=&-R-\frac{D}{2}\sum_{n=1}^{+\infty}ns_{\ n}^{(D)} \varphi^{n-1}+\frac{\left(D-1\right)\left(D+2\right)}{D-2}\left(\nabla \varphi\right)^{2}+\\
        &-\frac{D^{2}+4D-6}{D-2}\nabla^{2} \varphi+\mathcal{L}_{\xi} \varphi\ ,
    \end{split}
\end{equation}
where
\begin{equation}
        s_{\ k}^{(D)}\equiv\sum_{n=0}^{k}\frac{g_{n}}{\left(k-n\right)!n!}\left(\frac{2}{2-D}\right)^{k-n}\left(\frac{4D-6}{D-2}\right)^{n/2}\ .
\end{equation}
and:
\begin{equation}
    \left(g_1,\dots,g_{m-1},g_m,g_{m+1},g_{m+2},\dots\right)=\left(0,\dots,0,-\lambda,-\lambda,0,\dots\right)\ .
\end{equation}
In particular, given a positive integer $l>0$, we get:
\begin{equation}
    \begin{split}
        s_{\ m-l}^{(D)}=&0\ ,\\
        s_{\ m}^{(D)}=&-\frac{\lambda}{m!}\left(\frac{4D-6}{D-2}\right)^{m/2}\ ,\\
        s_{\ m+l}^{(D)}=&-\frac{\lambda}{m!l!}\left(\frac{2}{2-D}\right)^{l}\left(\frac{4D-6}{D-2}\right)^{m/2}+\\
        &\quad-\frac{\lambda}{(m+1)!(l-1)!}\left(\frac{2}{2-D}\right)^{l-1}\left(\frac{4D-6}{D-2}\right)^{(m+1)/2}\ .
    \end{split}
\end{equation}
Neglecting the diffeomorphisms, defining
\begin{equation}
    F\left(\varphi\right)\equiv\sum_{n=1}^{+\infty}ns_{\ n}^{(D)} \varphi^{n-1}
\end{equation}
and plugging-in the $\nabla_\mu\varphi=0$ condition, the flow equations reduce to:
\begin{equation}
        \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}-g_{\mu\nu}F\left(\varphi\right)\ ,\\
        \frac{\de \varphi}{\de\lambda}=&-R-\frac{D}{2}F\left(\varphi\right)\ .
    \end{split}
\end{equation}
The first equation, exploiting the fact that we work with an Einstein manifold, can be turned into a flow equation for $R$ as:
\begin{equation}
    \Dot{R}=2\frac{R^2}{D}+F\left(\varphi\right)R\ .
\end{equation}
Thus, in $D=4$, we have
\begin{equation}
            \begin{split}
        \Dot{R}=&\frac{R^2}{2}+F\left(\varphi\right)R\ ,\\
        \Dot{\varphi}=&-R-2F\left(\varphi\right)\ .
    \end{split}
\end{equation}
and:
\begin{equation}
    \begin{split}
        s_{m-l}=&0\ ,\quad s_{m}=-\frac{\lambda}{m!}\sqrt{5^{m}}\ ,\\
        s_{m+l}=&\frac{\left(-1\right)^{l}}{l!}\left[1-\frac{ l\sqrt{5}}{(m+1)}\right]s_{m}\ .
    \end{split}
\end{equation}
Defining the quantity
\begin{equation}
    \mathcal{A}\left(g,\varphi\right)\equiv R+2F\left(\varphi\right)\ ,
\end{equation}
the flow equations simplify as:
\begin{equation}
                \begin{split}
        \Dot{R}=&\frac{R}{2}\mathcal{A}\left(g,\varphi\right)\ ,\\
        \Dot{\varphi}=&-\mathcal{A}\left(g,\varphi\right)\ .
    \end{split}
\end{equation}
Writing things explicitly, we get
\begin{equation}
    \mathcal{A}\left(g,\varphi\right)=R-\lambda\varphi^{m-1}\sum_{l=0}^{\infty}c_{l}\varphi^l\ ,
\end{equation}
where we have introduced:
\begin{equation}
    c_l\equiv2\left(m+l\right)\frac{\left(-1\right)^l}{l!}\left(1-\frac{l\sqrt{5}}{m+1}\right)\frac{1}{m!}\sqrt{5^m}\ .
\end{equation}
First of all, we observe:
\begin{equation}
    \lim_{l\to\infty}c_l=0\ .
\end{equation}
Given the assumptions, the values of the Ricci curvature and the scalar are:
\begin{equation}
\varphi=-m\ ,\quad R=\lambda\frac{\left(-m\right)^m}{\left(m+1\right)!}\ .
\end{equation}
By expressing $\lambda$ in terms of $R$, we can finally write
\begin{equation}
     \mathcal{A}\left(g,\varphi\right)=R\left(1-\frac{15}{32}\varphi^{m-1}\sum_{l=0}^{\infty}c_{l}\varphi^l\right)\equiv R\cdot G\left(\varphi\right)\ ,
\end{equation}
and rephrase the flow equations as:
\begin{equation}
                \begin{split}
        \Dot{R}=&R^2\cdot G\left(\varphi\right)/2\ ,\\
        \Dot{\varphi}=&-R\cdot G\left(\varphi\right)\ .
    \end{split}
\end{equation}
\subsubsection{Fixed $m$}
At this point, we take $m=4$ and allow $\varphi$ to go off-shell along the flow. Namely, we drop its relation with $m$ except for the initial point. This way, we get:
\begin{equation}
    c_l\equiv\frac{\left(-1\right)^l}{l!}\left(1-\frac{l}{\sqrt{5}}\right)\frac{25\left(4+l\right)}{12}\ .
\end{equation}
As a starting point, we take $\lambda=1$.
    \begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Bubbles/Plotsream2.png}
    \caption{Plot of the vector field tangent to the flow, given generic initial conditions. In the above, the vertical axis corresponds to $\varphi$ while the horizontal one to $R$.}
\end{figure}
    \begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Bubbles/Plotstream.png}
    \caption{Plot of the vector field tangent to the flow, given the initial conditions $\varphi=-4$ and $R=32/15$. In the above, the vertical axis corresponds to $\varphi$ while the horizontal one to $R$.}
\end{figure}
As can be observed from the plot, starting from $\lambda=1$ and $m=4$, the system quickly goes to a fixed point.
\subsubsection{General analysis of the moduli space}
At this point, we take both $R$ and $\varphi$ to satisfy the on-shell conditions:
\begin{equation}
\varphi=-m\ ,\quad R=\lambda\frac{\left(-m\right)^m}{\left(m+1\right)!}\ .
\end{equation}
Being $R$ either positive (odd $m$) or negative (even $m$), the associated $4$-dimensional metric can always be written as
\begin{equation}
    \ds^2=\left(1-\frac{\Lambda r^2}{3}\right)\diff t^2+\left(1-\frac{\Lambda r^2}{3}\right)^{-1}\diff r^2+r^2\diff\Omega^2_2\ ,
\end{equation}
where the cosmological constant $\Lambda$ is:
\begin{equation}
    \Lambda=\frac{R}{4}=\frac{\lambda}{4}\frac{\left(-m\right)^m}{\left(m+1\right)!}\ .
\end{equation}
Now, we derive the entropy functional moving to the string frame version of the above action in $D=4$ as:
\begin{equation}
     \mathcal{F}=\int\diff^{D}x\sqrt{g}e^{-\varphi}\biggl[R+3\Delta \varphi+\left(\nabla \varphi\right)^2-\sum_{n=0}^{+\infty}s_{\ n}^{(D)}\varphi^{n}\biggr]\ .
\end{equation}
Plugging in the $\nabla_{\mu}\varphi=0$ condition and the expression for the metric and the scalar in terms of $m$ and $\lambda$, we have
\begin{equation}
\begin{split}
     \mathcal{F}\left[m,\lambda\right]&=-\int\diff^{4}x\ r^2\lambda\left(-m\right)^m e^{m}\biggl\{\frac{1}{\left(m+1\right)!}+\\
     &\quad+\frac{\sqrt{5^m}}{m!}\sum_{l=0}^{+\infty}\frac{m^{l}}{l!}\left[1-\frac{ l\sqrt{5}}{(m+1)}\right]\biggr\}=\\
     &\equiv\mathcal{T}\left(m,\lambda\right)\int\diff^{4}x\ r^2\ ,
\end{split}
\end{equation}
with:
\begin{equation}
    \mathcal{T}\left(m,\lambda\right)\equiv\lambda\left(-m\right)^m e^{m}\biggl\{\frac{1}{\left(m+1\right)!}+\frac{\sqrt{5^m}}{m!}\sum_{l=0}^{+\infty}\frac{m^{l}}{l!}\left[1-\frac{ l\sqrt{5}}{(m+1)}\right]\biggr\}\ .
\end{equation}
By inserting the above expression into the distance formula and assuming to start from a moduli space point with finite $\mathcal{T}$, we have:
\begin{equation}
    \Delta\sim|\log{\mathcal{T}\left(m,\lambda\right)}|\ .
\end{equation}
    \begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/Bubbles/Distance.png}
    \caption{Behaviour of the distance $\Delta$ in $m$, when $\lambda$ is fixed to $1$.}
\end{figure}
In order to study the $m\to\infty$ limit, we observe that:
\begin{equation}
    \lim_{m\to\infty}|\mathcal{T}\left(m,\lambda\right)|\sim\lambda m^m e^{2m}\frac{\sqrt{5^m}}{m!}\rightarrow\infty\ .
\end{equation}
Thus, the $m\to\infty$ limit lies at infinite distance. Similarly, the $\lambda\to\infty$ limit trivially lies too at $\infty$ distance. How can the two limits be interpreted? Looking, once more, at the \textit{reduced} action
\begin{equation}
    \mathcal{S}\left[g,\varphi\right]\equiv\int\diff^Dx\sqrt{g}\left[R+\frac{1}{2}\left(\nabla\varphi\right)^2+\frac{\lambda\varphi^{m}}{m!}+\frac{\lambda\varphi^{m+1}}{\left(m+1\right)!}\right]
\end{equation}
in the usual frame, we can straightforwardly observe that:
\begin{itemize}
    \item The $\lambda\to\infty$ limit is the \textit{strongly} coupled regime of the theory, where amplitudes diverge and the perturbative picture breaks down.
    \item The $m\to\infty$ limit is the \textit{high-order} limit of the interactions, in which all the allowed scalar vertices one should consider in computing scattering amplitudes involve infinitely many legs. 
\end{itemize}
\newpage




==> Theme/authorlist.tex <==
\noindent The following authors contributed to Chapter 1: Albert Einstein, George Gamow and Pief Panofsky.

\noindent The following authors contributed to Chapter 2: I. I. Rabi, Niels Bohr and Norman Ramsey.

\noindent The following authors contributed to Chapter 3: Ramon y Cajal, Andrew Huxley.

==> Theme/colophon.tex <==
\newpage

% If you do want an image in the colophon:
\begin{figure}
  \vspace{50pt}
  \centering
    \includegraphics[width=0.51\textwidth]{endmatter/colophon.png}
\end{figure}

% If you don't want an image in the colophon:
% \vspace*{200pt}

\begin{center}
\parbox{200pt}{\lettrine[lines=3,slope=-2pt,nindent=-4pt]{\textcolor{SchoolColor}{T}}{his thesis was typeset} using \LaTeX, originally developed by Leslie Lamport and based on Donald Knuth's \TeX. The body text is set in 11 point Egenolff-Berner Garamond, a revival of Claude Garamont's humanist typeface. The above illustration, ``Science Experiment 02'', was created by Ben Schlitter and released under \href{http://creativecommons.org/licenses/by-nc-nd/3.0/}{\textsc{cc by-nc-nd 3.0}}. A template that can be used to format a PhD thesis with this look and feel has been released under the permissive \textsc{mit} (\textsc{x}11) license, and can be found online at \href{https://github.com/suchow/Dissertate}{github.com/suchow/Dissertate} or from its author, Jordan Suchow, at \href{mailto:suchow@post.harvard.edu}{suchow@post.harvard.edu}.}
\end{center}

==> circle.tex <==
\textbf{ }\\
\textbf{ }\\
\textbf{ }\\
\textbf{ }\\
\textbf{ }\\
\textbf{ }\\
\begin{center}
\begin{figure}[h]
\centering
\includegraphics[width=0.15\linewidth]{Figures/Arrow.png}
\label{}
\end{figure}
\end{center}
